Impact of Evaluation Methodologies on Code Summarization

There has been a growing interest in developing machine learning (ML) models for code summarization tasks, e.g., comment generation and method naming. Despite substantial increase in the effectiveness of ML models, the evaluation methodologies, i.e., the way people split datasets into training, validation, and test sets, were not well studied. Specifically, no prior work on code summarization considered the timestamps of code and comments during evaluation. This may lead to evaluations that are inconsistent with the intended use cases. In this paper, we introduce the time-segmented evaluation methodology, which is novel to the code summarization research community, and compare it with the mixed-project and cross-project methodologies that have been commonly used. Each methodology can be mapped to some use cases, and the time-segmented methodology should be adopted in the evaluation of ML models for code summarization. To assess the impact of methodologies, we collect a dataset of (code, comment) pairs with timestamps to train and evaluate several recent ML models for code summarization. Our experiments show that different methodologies lead to conflicting evaluation results. We invite the community to expand the set of methodologies used in evaluations.

==> code/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%% ==========
%%% Highlight code line

\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
  \begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
}
\def\bt@HL@endenv{%
  \end{btHighlight}%
  \egroup
}
\newcommand{\bt@HL@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=1pt, inner ysep=0pt, rounded corners=1pt, minimum height=\ht\strutbox,#1]{\raisebox{1pt}{\strut}\strut\usebox{#2}};
  }%
}

\newenvironment{btHighlightLine}[1][]
{\begingroup\tikzset{bt@HighlightLine@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HLLine@box[bt@HighlightLine@par]{\@tempboxa}\endgroup}

\newcommand\btHLLine[1][]{%
  \begin{btHighlightLine}[#1]\bgroup\aftergroup\bt@HLLine@endenv%
}
\def\bt@HLLine@endenv{%
  \end{btHighlightLine}%
  \egroup
}
\newcommand{\bt@HLLine@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{0pt}{-1pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=0pt, inner ysep=0pt, minimum height=\ht\strutbox+3pt, minimum width=\linewidth,#1] (line-bg) {};
    \node[right = 0 of line-bg.west, outer sep=0pt, inner xsep=0pt, inner ysep=0pt]{\raisebox{0pt}{\strut}\strut\usebox{#2}};
  }%
}
\makeatother

% Disable tikz's error message complaining redefining dollor-sign.  WARNING: this may indeed cause problems but hopefully not
\makeatletter
\global\let\tikz@ensure@dollar@catcode=\relax
\makeatother


%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=6pt,
  numbersep=2pt,
  showstringspaces=false,
  moredelim=**[il][{\btHLLine[fill=blue!10]}]{<HLL/>},
  moredelim=**[is][{\btHL[fill=blue!20]}]{<HL>}{<HL/>},
}

\lstset{escapeinside={(*@}{@*)}}

\newcommand{\JavaIn}[1]{\lstinline[language=java-pretty]{#1}}

%%%==========


==> code/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> figs/dataset-MN/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|c|c|c || l|c|}
\hline
& \textbf{ATrain} & \textbf{\AVal} & \textbf{\ATestS} & & \textbf{\ATestC} \\
\hline
\UseMacro{TH-ds-MP}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/train-MP}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/val-MP}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_standard-MP}\end{minipage}
 & \UseMacro{TH-ds-MP-CP}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_common-MP-CP}\end{minipage}
\\
\hline
\UseMacro{TH-ds-CP}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/train-CP}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/val-CP}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_standard-CP}\end{minipage}
 & \UseMacro{TH-ds-MP-T}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_common-MP-T}\end{minipage}
\\
\hline
\UseMacro{TH-ds-T}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/train-T}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/val-T}\end{minipage}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_standard-T}\end{minipage}
 & \UseMacro{TH-ds-CP-T}
 & \begin{minipage}{.18\textwidth}\includegraphics[width=\textwidth]{figs/dataset-MN/test_common-CP-T}\end{minipage}
\\
\hline
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_standard-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_standard-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_standard-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-CP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-CP-T-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-CP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-CP-T-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-CP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-CP-T-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_same_code/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_standard-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_standard-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_standard-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_same_code/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_same_code/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-CP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-CP-T-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-CP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-CP-T-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-CP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-CP-T-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_code/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_same_code/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_same_nl/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_standard-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_standard-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_standard-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_same_nl/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_same_nl/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-CP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-CP-T-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-CP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-CP-T-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-CP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-CP-T-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_same_nl/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_same_nl/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_sim_90/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_standard-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-val-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_standard-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_standard-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-val-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_standard-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_standard-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-val-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_standard-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_sim_90/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-CG_nd_sim_90/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-bleu}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-MP-CP-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-MP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-CP-T-bleu}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-CP-T-bleu}\end{minipage}
\\
\UseMacro{TH-metric-meteor}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-MP-CP-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-MP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-CP-T-meteor}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-CP-T-meteor}\end{minipage}
\\
\UseMacro{TH-metric-rouge_l_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-MP-CP-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-MP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-CP-T-rouge_l_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-CP-T-rouge_l_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-CG_nd_sim_90/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-CG_nd_sim_90/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_standard-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_standard-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_standard-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-CP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-CP-T-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-CP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-CP-T-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-CP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-CP-T-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_same_code/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_standard-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_standard-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_standard-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_same_code/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_same_code/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-CP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-CP-T-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-CP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-CP-T-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-CP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-CP-T-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_code/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_same_code/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_same_nl/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_standard-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_standard-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_standard-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_same_nl/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_same_nl/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-CP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-CP-T-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-CP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-CP-T-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-CP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-CP-T-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_same_nl/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_same_nl/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_sim_90/plot-aux.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|c|c|c|c|c|c|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_standard-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-val-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_standard-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_standard-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-val-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_standard-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_standard-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-val-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_standard-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_standard-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-val-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_standard-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_sim_90/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> figs/results-MN_nd_sim_90/plot.tex <==

%% Automatically generated by pyutil.latex 

\begin{center}
\begin{footnotesize}
\begin{tabular}{|r|@{}c@{}c@{}|@{}c@{}c@{}|@{}c@{}c@{}|}
\hline
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\
\hline
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP-T}}
\\
\hline
\UseMacro{TH-metric-set_match_p}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-MP-CP-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-MP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-CP-T-set_match_p}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-CP-T-set_match_p}\end{minipage}
\\
\UseMacro{TH-metric-set_match_r}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-MP-CP-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-MP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-CP-T-set_match_r}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-CP-T-set_match_r}\end{minipage}
\\
\UseMacro{TH-metric-set_match_f}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-MP-CP-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-MP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-CP-T-set_match_f}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-CP-T-set_match_f}\end{minipage}
\\
\UseMacro{TH-metric-exact_match}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-MP-CP-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-MP-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-MP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-CP-test_common-CP-T-exact_match}\end{minipage}
 & \begin{minipage}{.12\textwidth}\includegraphics[width=\textwidth]{figs/results-MN_nd_sim_90/bar-T-test_common-CP-T-exact_match}\end{minipage}
\\
\hline
\multicolumn{7}{c}{\includegraphics[scale=0.3]{figs/results-MN_nd_sim_90/legend}} \\
\end{tabular}
\end{footnotesize}
\end{center}


==> tables/CG_nd_same_code/numbers-results-CG.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_same_code}{10.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_same_code}{1.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_same_code}{17.2}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_code}{22.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_p_same_code}{24.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_r_same_code}{25.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_same_code}{10.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_code}{0.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_same_code}{17.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_code}{22.8}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_same_code}{24.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_same_code}{24.9}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_same_code}{10.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_same_code}{0.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_same_code}{17.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_same_code}{23.2}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_p_same_code}{24.9}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_r_same_code}{25.5}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_same_code}{12.5}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_same_code}{0.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_same_code}{20.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_same_code}{28.0}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_p_same_code}{35.3}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_r_same_code}{26.2}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_same_code}{12.6}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_same_code}{0.6}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_same_code}{19.9}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_code}{28.2}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_p_same_code}{35.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_r_same_code}{26.1}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_bleu_same_code}{13.0}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_same_code}{0.7}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_meteor_same_code}{20.5}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_same_code}{28.9}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_p_same_code}{36.4}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_r_same_code}{26.9}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_same_code}{13.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_same_code}{1.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_same_code}{20.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_same_code}{29.0}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_p_same_code}{38.0}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_r_same_code}{26.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_same_code}{12.9}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_same_code}{0.8}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_same_code}{20.0}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_code}{29.0}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_p_same_code}{38.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_r_same_code}{25.9}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_bleu_same_code}{13.3}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_same_code}{1.0}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_meteor_same_code}{20.3}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_same_code}{29.4}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_p_same_code}{38.6}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_r_same_code}{26.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_same_code}{37.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_code}{22.4}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_same_code}{46.4}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_code}{51.0}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_same_code}{52.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_same_code}{52.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_same_code}{48.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_same_code}{36.1}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_same_code}{55.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_code}{59.3}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_p_same_code}{60.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_r_same_code}{60.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_same_code}{42.3}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_same_code}{27.2}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_same_code}{50.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_same_code}{54.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_p_same_code}{56.1}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_r_same_code}{56.6}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_same_code}{48.7}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_same_code}{31.5}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_same_code}{57.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_code}{62.6}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_p_same_code}{67.0}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_r_same_code}{61.5}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_same_code}{59.2}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_same_code}{46.6}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_same_code}{65.5}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_same_code}{69.7}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_p_same_code}{73.1}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_r_same_code}{68.9}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_bleu_same_code}{53.6}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_same_code}{37.9}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_meteor_same_code}{61.6}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_same_code}{66.1}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_p_same_code}{69.9}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_r_same_code}{65.4}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_same_code}{52.8}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_same_code}{34.7}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_same_code}{61.5}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_code}{66.1}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_p_same_code}{69.9}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_r_same_code}{65.2}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_same_code}{63.2}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_same_code}{50.4}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_same_code}{69.3}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_same_code}{72.8}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_p_same_code}{75.7}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_r_same_code}{72.2}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_bleu_same_code}{57.6}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_same_code}{41.0}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_meteor_same_code}{65.6}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_same_code}{69.5}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_p_same_code}{72.6}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_r_same_code}{69.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_same_code}{36.8}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_same_code}{26.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_same_code}{44.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_code}{48.5}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_p_same_code}{50.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_r_same_code}{50.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_same_code}{38.5}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_same_code}{26.8}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_same_code}{45.5}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_code}{49.6}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_p_same_code}{50.5}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_r_same_code}{52.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_same_code}{38.9}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_same_code}{27.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_same_code}{46.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_same_code}{50.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_p_same_code}{51.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_r_same_code}{52.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_same_code}{46.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_same_code}{35.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_same_code}{53.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_same_code}{58.6}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_p_same_code}{63.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_r_same_code}{57.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_same_code}{50.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_same_code}{38.9}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_same_code}{56.9}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_same_code}{61.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_p_same_code}{64.9}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_r_same_code}{61.1}
\DefMacro{result-CG_T_RNNBaseline_test_standard_bleu_same_code}{50.2}
\DefMacro{result-CG_T_RNNBaseline_test_standard_exact_match_same_code}{38.5}
\DefMacro{result-CG_T_RNNBaseline_test_standard_meteor_same_code}{56.7}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_same_code}{61.3}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_p_same_code}{64.9}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_r_same_code}{60.9}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_same_code}{49.1}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_same_code}{38.2}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_same_code}{55.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_same_code}{60.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_p_same_code}{65.3}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_r_same_code}{59.5}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_same_code}{53.5}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_same_code}{41.9}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_same_code}{59.9}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_same_code}{63.9}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_p_same_code}{66.9}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_r_same_code}{63.7}
\DefMacro{result-CG_T_TransformerACL20_test_standard_bleu_same_code}{53.6}
\DefMacro{result-CG_T_TransformerACL20_test_standard_exact_match_same_code}{42.0}
\DefMacro{result-CG_T_TransformerACL20_test_standard_meteor_same_code}{60.0}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_same_code}{64.2}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_p_same_code}{67.3}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_r_same_code}{63.9}


==> tables/CG_nd_same_code/table-results-CG_same_code.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_same_code}
 & $^{\beta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_same_code}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_same_code}
 & $^{\beta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_same_code}}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_same_code}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_same_code}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_same_code}
 & $^{\delta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_same_code}
 & $^{\gamma}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_same_code}
 & $^{\delta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_same_code}
 & $^{\epsilon}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_same_code}}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_same_code}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_same_code}}
 & $^{\epsilon}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_code}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_code}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_same_code}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_code}
 & $^{\zeta}$$^{\eta}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_same_code}
 & $^{\iota}$$^{\kappa}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_same_code}
 & $^{\zeta}$$^{\theta}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_same_code}
 & $^{\iota}$$^{\lambda}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_same_code}}
 & $^{\eta}$$^{\theta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_same_code}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_same_code}}
 & $^{\kappa}$$^{\lambda}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_same_code}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_same_code}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-CG_same_code}}
\caption{\UseMacro{TC-results-CG_same_code}}
\end{table}


==> tables/CG_nd_same_code/table-results-aux-CG_same_code.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_bleu_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_bleu_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_bleu_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_bleu_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_bleu_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_val_bleu_same_code}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_bleu_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_val_bleu_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_bleu_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_bleu_same_code}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_bleu_same_code}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_bleu_same_code}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_bleu_same_code}}
 & \UseMacro{result-CG_T_TransformerACL20_val_bleu_same_code}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_bleu_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_meteor_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_meteor_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_meteor_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_meteor_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_meteor_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_val_meteor_same_code}
 & $^{\beta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_standard_meteor_same_code}}
 & \UseMacro{result-CG_T_RNNBaseline_val_meteor_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_meteor_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_meteor_same_code}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_meteor_same_code}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_meteor_same_code}
 & $^{\beta}$\UseMacro{result-CG_CP_TransformerACL20_test_standard_meteor_same_code}
 & \UseMacro{result-CG_T_TransformerACL20_val_meteor_same_code}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_meteor_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_rouge_l_f_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_rouge_l_f_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_val_rouge_l_f_same_code}
 & $^{\gamma}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_val_rouge_l_f_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_rouge_l_f_same_code}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_same_code}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_rouge_l_f_same_code}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_same_code}}
 & \UseMacro{result-CG_T_TransformerACL20_val_rouge_l_f_same_code}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_same_code}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_exact_match_same_code}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_same_code}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_exact_match_same_code}
 & $^{\delta}$$^{\epsilon}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_exact_match_same_code}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_same_code}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_exact_match_same_code}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_same_code}
 & \UseMacro{result-CG_CP_RNNBaseline_val_exact_match_same_code}
 & $^{\delta}$$^{\zeta}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_val_exact_match_same_code}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_exact_match_same_code}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_exact_match_same_code}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_same_code}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_exact_match_same_code}
 & $^{\epsilon}$$^{\zeta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_same_code}}
 & \UseMacro{result-CG_T_TransformerACL20_val_exact_match_same_code}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_exact_match_same_code}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-CG_same_code}}
\caption{\UseMacro{TC-results-aux-CG_same_code}}
\end{table}


==> tables/CG_nd_same_nl/numbers-results-CG.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_same_nl}{9.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_same_nl}{0.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_same_nl}{16.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_nl}{22.3}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_p_same_nl}{24.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_r_same_nl}{23.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_same_nl}{10.2}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_nl}{0.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_same_nl}{17.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_nl}{23.3}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_same_nl}{25.6}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_same_nl}{25.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_same_nl}{10.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_same_nl}{0.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_same_nl}{17.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}{22.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_p_same_nl}{24.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_r_same_nl}{25.0}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_same_nl}{11.3}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_same_nl}{0.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_same_nl}{19.6}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_same_nl}{28.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_p_same_nl}{36.7}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_r_same_nl}{25.4}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_same_nl}{12.6}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_same_nl}{0.3}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_same_nl}{20.2}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_nl}{28.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_p_same_nl}{37.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_r_same_nl}{26.1}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_bleu_same_nl}{12.5}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_same_nl}{0.2}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_meteor_same_nl}{20.0}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_same_nl}{28.4}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_p_same_nl}{36.0}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_r_same_nl}{26.5}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_same_nl}{11.6}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_same_nl}{0.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_same_nl}{19.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_same_nl}{28.7}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_p_same_nl}{38.9}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_r_same_nl}{25.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_same_nl}{12.6}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_same_nl}{0.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_same_nl}{20.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_nl}{29.7}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_p_same_nl}{39.5}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_r_same_nl}{26.2}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_bleu_same_nl}{12.6}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_same_nl}{0.3}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_meteor_same_nl}{19.6}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_same_nl}{28.8}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_p_same_nl}{38.1}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_r_same_nl}{25.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_same_nl}{20.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_nl}{1.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_same_nl}{31.4}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_nl}{37.3}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_same_nl}{39.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_same_nl}{38.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_same_nl}{20.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_same_nl}{2.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_same_nl}{30.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_nl}{35.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_p_same_nl}{38.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_r_same_nl}{37.4}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_same_nl}{22.2}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_same_nl}{2.8}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_same_nl}{33.0}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}{38.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_p_same_nl}{40.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_r_same_nl}{40.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_same_nl}{29.3}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_same_nl}{6.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_same_nl}{41.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_nl}{48.2}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_p_same_nl}{53.9}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_r_same_nl}{46.9}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_same_nl}{27.5}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_same_nl}{7.0}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_same_nl}{38.6}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_same_nl}{45.2}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_p_same_nl}{51.7}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_r_same_nl}{43.7}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_bleu_same_nl}{31.2}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_same_nl}{8.7}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_meteor_same_nl}{43.3}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_same_nl}{49.5}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_p_same_nl}{54.7}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_r_same_nl}{48.5}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_same_nl}{32.9}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_same_nl}{7.6}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_same_nl}{45.2}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_nl}{51.6}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_p_same_nl}{57.0}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_r_same_nl}{50.3}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_same_nl}{30.5}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_same_nl}{7.4}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_same_nl}{42.0}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_same_nl}{48.3}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_p_same_nl}{54.4}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_r_same_nl}{47.0}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_bleu_same_nl}{34.4}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_same_nl}{9.9}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_meteor_same_nl}{46.9}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_same_nl}{52.7}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_p_same_nl}{57.6}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_r_same_nl}{51.8}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_same_nl}{13.2}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_same_nl}{0.4}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_same_nl}{21.4}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_nl}{27.6}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_p_same_nl}{30.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_r_same_nl}{29.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_same_nl}{15.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_same_nl}{0.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_same_nl}{23.6}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_nl}{29.3}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_p_same_nl}{31.4}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_r_same_nl}{31.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_same_nl}{15.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_same_nl}{0.2}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_same_nl}{23.9}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}{29.7}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_p_same_nl}{31.6}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_r_same_nl}{31.8}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_same_nl}{16.7}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_same_nl}{1.0}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_same_nl}{27.1}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_same_nl}{34.5}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_p_same_nl}{41.0}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_r_same_nl}{32.9}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_same_nl}{18.6}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_same_nl}{0.7}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_same_nl}{29.1}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_same_nl}{36.0}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_p_same_nl}{42.6}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_r_same_nl}{34.7}
\DefMacro{result-CG_T_RNNBaseline_test_standard_bleu_same_nl}{19.2}
\DefMacro{result-CG_T_RNNBaseline_test_standard_exact_match_same_nl}{1.0}
\DefMacro{result-CG_T_RNNBaseline_test_standard_meteor_same_nl}{29.4}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_same_nl}{36.7}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_p_same_nl}{42.6}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_r_same_nl}{35.6}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_same_nl}{17.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_same_nl}{1.2}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_same_nl}{28.4}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_same_nl}{36.0}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_p_same_nl}{43.0}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_r_same_nl}{34.1}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_same_nl}{19.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_same_nl}{1.1}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_same_nl}{30.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_same_nl}{37.4}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_p_same_nl}{43.8}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_r_same_nl}{36.1}
\DefMacro{result-CG_T_TransformerACL20_test_standard_bleu_same_nl}{20.7}
\DefMacro{result-CG_T_TransformerACL20_test_standard_exact_match_same_nl}{1.5}
\DefMacro{result-CG_T_TransformerACL20_test_standard_meteor_same_nl}{31.7}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_same_nl}{38.8}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_p_same_nl}{44.7}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_r_same_nl}{37.7}


==> tables/CG_nd_same_nl/table-results-CG_same_nl.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_same_nl}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_same_nl}}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_same_nl}
 & $^{\beta}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_same_nl}}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_same_nl}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_same_nl}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_same_nl}}
 & $^{\beta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_same_nl}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_same_nl}
 & $^{\delta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_same_nl}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_same_nl}}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_same_nl}
 & $^{\epsilon}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_same_nl}}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_same_nl}}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_same_nl}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_same_nl}}
 & $^{\delta}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_same_nl}}
 & $^{\epsilon}$\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_same_nl}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_same_nl}
 & $^{\zeta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_nl}
 & $^{\theta}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_same_nl}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_same_nl}
 & $^{\zeta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_same_nl}
 & $^{\eta}$$^{\theta}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_nl}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_same_nl}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_same_nl}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_same_nl}}
 & $^{\eta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_same_nl}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_nl}
 & $^{\iota}$$^{\kappa}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_same_nl}
 & $^{\tau}$$^{\pi}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_same_nl}
 & $^{\sigma}$$^{\tau}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_same_nl}
 & $^{\iota}$$^{\lambda}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_same_nl}}
 & $^{\mu}$\UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_same_nl}
 & $^{\nu}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_same_nl}
 & $^{\tau}$$^{\rho}$$^{\sigma}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_same_nl}
 & $^{\upsilon}$\UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_same_nl}}
 & $^{\kappa}$$^{\lambda}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_same_nl}}
 & $^{\mu}$\textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_same_nl}}
 & $^{\nu}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_same_nl}}
 & $^{\pi}$$^{\rho}$$^{\tau}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_same_nl}}
 & $^{\upsilon}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_same_nl}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-CG_same_nl}}
\caption{\UseMacro{TC-results-CG_same_nl}}
\end{table}


==> tables/CG_nd_same_nl/table-results-aux-CG_same_nl.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_bleu_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_bleu_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_bleu_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_bleu_same_nl}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_bleu_same_nl}
 & \UseMacro{result-CG_CP_RNNBaseline_val_bleu_same_nl}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_bleu_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_val_bleu_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_bleu_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_bleu_same_nl}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_bleu_same_nl}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_bleu_same_nl}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_bleu_same_nl}}
 & \UseMacro{result-CG_T_TransformerACL20_val_bleu_same_nl}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_bleu_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_meteor_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_meteor_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_meteor_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_meteor_same_nl}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_meteor_same_nl}
 & \UseMacro{result-CG_CP_RNNBaseline_val_meteor_same_nl}
 & $^{\beta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_standard_meteor_same_nl}}
 & \UseMacro{result-CG_T_RNNBaseline_val_meteor_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_meteor_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_meteor_same_nl}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_meteor_same_nl}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_meteor_same_nl}
 & $^{\beta}$\UseMacro{result-CG_CP_TransformerACL20_test_standard_meteor_same_nl}
 & \UseMacro{result-CG_T_TransformerACL20_val_meteor_same_nl}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_meteor_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_rouge_l_f_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_rouge_l_f_same_nl}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_same_nl}
 & \UseMacro{result-CG_CP_RNNBaseline_val_rouge_l_f_same_nl}
 & $^{\gamma}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_val_rouge_l_f_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_rouge_l_f_same_nl}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_same_nl}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_rouge_l_f_same_nl}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_same_nl}}
 & \UseMacro{result-CG_T_TransformerACL20_val_rouge_l_f_same_nl}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_exact_match_same_nl}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_same_nl}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_exact_match_same_nl}
 & $^{\delta}$$^{\epsilon}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_exact_match_same_nl}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_same_nl}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_exact_match_same_nl}
 & $^{\eta}$\UseMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_same_nl}
 & \UseMacro{result-CG_CP_RNNBaseline_val_exact_match_same_nl}
 & $^{\delta}$$^{\zeta}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_same_nl}
 & \UseMacro{result-CG_T_RNNBaseline_val_exact_match_same_nl}
 & $^{\theta}$\UseMacro{result-CG_T_RNNBaseline_test_standard_exact_match_same_nl}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_exact_match_same_nl}
 & $^{\eta}$\textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_same_nl}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_exact_match_same_nl}
 & $^{\epsilon}$$^{\zeta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_same_nl}}
 & \UseMacro{result-CG_T_TransformerACL20_val_exact_match_same_nl}
 & $^{\theta}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_exact_match_same_nl}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-CG_same_nl}}
\caption{\UseMacro{TC-results-aux-CG_same_nl}}
\end{table}


==> tables/CG_nd_sim_90/numbers-results-CG.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_sim_90}{9.5}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_sim_90}{0.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_sim_90}{16.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_sim_90}{22.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_p_sim_90}{24.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_r_sim_90}{23.9}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_sim_90}{10.3}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_sim_90}{0.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_sim_90}{17.3}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_sim_90}{23.2}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_sim_90}{25.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_sim_90}{25.1}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_sim_90}{10.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_sim_90}{0.0}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_sim_90}{16.7}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}{22.4}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_p_sim_90}{24.2}
\DefMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_r_sim_90}{24.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_sim_90}{11.6}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_sim_90}{0.2}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_sim_90}{20.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_sim_90}{28.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_p_sim_90}{37.2}
\DefMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_r_sim_90}{26.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_sim_90}{13.0}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_sim_90}{0.3}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_sim_90}{20.8}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_sim_90}{29.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_p_sim_90}{37.1}
\DefMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_r_sim_90}{26.7}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_bleu_sim_90}{12.4}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_sim_90}{0.2}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_meteor_sim_90}{19.9}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_sim_90}{28.3}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_p_sim_90}{35.8}
\DefMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_r_sim_90}{26.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_sim_90}{11.6}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_sim_90}{0.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_sim_90}{19.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_sim_90}{28.7}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_p_sim_90}{38.9}
\DefMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_r_sim_90}{25.2}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_sim_90}{13.1}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_sim_90}{0.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_sim_90}{20.8}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_sim_90}{29.9}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_p_sim_90}{39.3}
\DefMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_r_sim_90}{26.7}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_bleu_sim_90}{12.5}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_sim_90}{0.3}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_meteor_sim_90}{19.4}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_sim_90}{28.6}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_p_sim_90}{37.9}
\DefMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_r_sim_90}{25.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_sim_90}{16.3}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_sim_90}{0.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_sim_90}{26.1}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_sim_90}{32.2}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_p_sim_90}{34.2}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_r_sim_90}{34.3}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_sim_90}{13.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_sim_90}{0.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_sim_90}{22.1}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_sim_90}{27.6}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_p_sim_90}{29.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_r_sim_90}{29.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_sim_90}{16.9}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_sim_90}{1.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_sim_90}{27.0}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}{32.7}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_p_sim_90}{34.5}
\DefMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_r_sim_90}{35.1}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_sim_90}{24.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_sim_90}{4.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_sim_90}{36.1}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_sim_90}{43.4}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_p_sim_90}{49.3}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_r_sim_90}{42.1}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_sim_90}{19.2}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_sim_90}{2.2}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_sim_90}{29.9}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_sim_90}{37.0}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_p_sim_90}{43.5}
\DefMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_r_sim_90}{35.6}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_bleu_sim_90}{25.4}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_sim_90}{5.9}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_meteor_sim_90}{37.3}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_sim_90}{44.0}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_p_sim_90}{49.5}
\DefMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_r_sim_90}{43.1}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_sim_90}{26.8}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_sim_90}{5.3}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_sim_90}{39.1}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_sim_90}{46.0}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_p_sim_90}{51.9}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_r_sim_90}{44.7}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_sim_90}{21.4}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_sim_90}{2.2}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_sim_90}{32.5}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_sim_90}{39.6}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_p_sim_90}{45.9}
\DefMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_r_sim_90}{38.2}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_bleu_sim_90}{27.8}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_sim_90}{6.8}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_meteor_sim_90}{40.3}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_sim_90}{46.7}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_p_sim_90}{51.9}
\DefMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_r_sim_90}{45.8}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_sim_90}{11.2}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_sim_90}{0.4}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_sim_90}{19.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_sim_90}{25.4}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_p_sim_90}{27.8}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_r_sim_90}{26.9}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_sim_90}{10.7}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_sim_90}{0.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_sim_90}{18.2}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_sim_90}{23.6}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_p_sim_90}{25.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_r_sim_90}{26.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_sim_90}{12.0}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_sim_90}{0.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_sim_90}{20.1}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}{25.9}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_p_sim_90}{27.5}
\DefMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_r_sim_90}{28.5}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_sim_90}{14.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_sim_90}{0.9}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_sim_90}{24.4}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_sim_90}{32.2}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_p_sim_90}{38.8}
\DefMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_r_sim_90}{30.5}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_sim_90}{13.8}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_sim_90}{0.1}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_sim_90}{23.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_sim_90}{30.3}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_p_sim_90}{36.7}
\DefMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_r_sim_90}{29.3}
\DefMacro{result-CG_T_RNNBaseline_test_standard_bleu_sim_90}{16.0}
\DefMacro{result-CG_T_RNNBaseline_test_standard_exact_match_sim_90}{0.8}
\DefMacro{result-CG_T_RNNBaseline_test_standard_meteor_sim_90}{25.6}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_sim_90}{33.1}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_p_sim_90}{38.8}
\DefMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_r_sim_90}{32.2}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_sim_90}{15.1}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_sim_90}{1.2}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_sim_90}{25.4}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_sim_90}{33.3}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_p_sim_90}{40.5}
\DefMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_r_sim_90}{31.4}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_sim_90}{14.6}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_sim_90}{0.1}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_sim_90}{24.5}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_sim_90}{31.6}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_p_sim_90}{37.7}
\DefMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_r_sim_90}{30.5}
\DefMacro{result-CG_T_TransformerACL20_test_standard_bleu_sim_90}{17.2}
\DefMacro{result-CG_T_TransformerACL20_test_standard_exact_match_sim_90}{1.2}
\DefMacro{result-CG_T_TransformerACL20_test_standard_meteor_sim_90}{27.7}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_sim_90}{35.0}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_p_sim_90}{40.8}
\DefMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_r_sim_90}{34.0}


==> tables/CG_nd_sim_90/table-results-CG_sim_90.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu_sim_90}
 & $^{\beta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu_sim_90}
 & $^{\delta}$$^{\epsilon}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu_sim_90}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu_sim_90}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu_sim_90}
 & $^{\beta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu_sim_90}
 & $^{\gamma}$$^{\delta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu_sim_90}}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu_sim_90}}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu_sim_90}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu_sim_90}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu_sim_90}}
 & $^{\gamma}$$^{\epsilon}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu_sim_90}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor_sim_90}
 & $^{\eta}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor_sim_90}
 & $^{\zeta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor_sim_90}}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor_sim_90}
 & \textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor_sim_90}}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor_sim_90}}
 & $^{\zeta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor_sim_90}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor_sim_90}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor_sim_90}}
 & $^{\eta}$\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor_sim_90}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f_sim_90}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f_sim_90}
 & $^{\theta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f_sim_90}}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f_sim_90}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f_sim_90}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f_sim_90}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f_sim_90}}
 & $^{\theta}$\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f_sim_90}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match_sim_90}
 & $^{\iota}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match_sim_90}
 & $^{\nu}$$^{\tau}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match_sim_90}
 & $^{\rho}$$^{\sigma}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match_sim_90}
 & $^{\upsilon}$$^{\phi}$\UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & $^{\lambda}$\UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match_sim_90}
 & $^{\iota}$$^{\kappa}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match_sim_90}}
 & $^{\mu}$\textbf{\UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match_sim_90}}
 & $^{\nu}$$^{\pi}$\textbf{\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match_sim_90}}
 & $^{\rho}$$^{\tau}$$^{\upsilon}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match_sim_90}}
 & $^{\chi}$\UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & $^{\lambda}$\textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match_sim_90}}
 & $^{\kappa}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match_sim_90}}
 & $^{\mu}$\textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match_sim_90}}
 & $^{\tau}$$^{\pi}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match_sim_90}}
 & $^{\sigma}$$^{\tau}$$^{\phi}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match_sim_90}}
 & $^{\chi}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match_sim_90}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-CG_sim_90}}
\caption{\UseMacro{TC-results-CG_sim_90}}
\end{table}


==> tables/CG_nd_sim_90/table-results-aux-CG_sim_90.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_bleu_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_bleu_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_bleu_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_bleu_sim_90}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_bleu_sim_90}
 & \UseMacro{result-CG_CP_RNNBaseline_val_bleu_sim_90}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_bleu_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_val_bleu_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_bleu_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_bleu_sim_90}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_bleu_sim_90}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_bleu_sim_90}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_bleu_sim_90}}
 & \UseMacro{result-CG_T_TransformerACL20_val_bleu_sim_90}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_bleu_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_meteor_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_meteor_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_meteor_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_meteor_sim_90}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_meteor_sim_90}
 & \UseMacro{result-CG_CP_RNNBaseline_val_meteor_sim_90}
 & $^{\beta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_standard_meteor_sim_90}}
 & \UseMacro{result-CG_T_RNNBaseline_val_meteor_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_meteor_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_meteor_sim_90}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_meteor_sim_90}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_meteor_sim_90}
 & $^{\beta}$\UseMacro{result-CG_CP_TransformerACL20_test_standard_meteor_sim_90}
 & \UseMacro{result-CG_T_TransformerACL20_val_meteor_sim_90}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_meteor_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_rouge_l_f_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_rouge_l_f_sim_90}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f_sim_90}
 & \UseMacro{result-CG_CP_RNNBaseline_val_rouge_l_f_sim_90}
 & $^{\gamma}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_val_rouge_l_f_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_rouge_l_f_sim_90}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f_sim_90}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_rouge_l_f_sim_90}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f_sim_90}}
 & \UseMacro{result-CG_T_TransformerACL20_val_rouge_l_f_sim_90}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_exact_match_sim_90}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match_sim_90}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_exact_match_sim_90}
 & $^{\delta}$$^{\epsilon}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_exact_match_sim_90}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match_sim_90}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_exact_match_sim_90}
 & $^{\eta}$\UseMacro{result-CG_MP_RNNBaseline_test_standard_exact_match_sim_90}
 & \UseMacro{result-CG_CP_RNNBaseline_val_exact_match_sim_90}
 & $^{\delta}$$^{\zeta}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_exact_match_sim_90}
 & \UseMacro{result-CG_T_RNNBaseline_val_exact_match_sim_90}
 & $^{\theta}$\UseMacro{result-CG_T_RNNBaseline_test_standard_exact_match_sim_90}
\\
\UseMacro{TH-model-TransformerACL20}
 & \UseMacro{result-CG_MP_TransformerACL20_val_exact_match_sim_90}
 & $^{\eta}$\textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_exact_match_sim_90}}
 & \UseMacro{result-CG_CP_TransformerACL20_val_exact_match_sim_90}
 & $^{\epsilon}$$^{\zeta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_exact_match_sim_90}}
 & \UseMacro{result-CG_T_TransformerACL20_val_exact_match_sim_90}
 & $^{\theta}$\textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_exact_match_sim_90}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-CG_sim_90}}
\caption{\UseMacro{TC-results-aux-CG_sim_90}}
\end{table}


==> tables/MN_nd_same_code/numbers-results-MN.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_same_code}{5.7}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_same_code}{28.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_same_code}{34.5}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_same_code}{25.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_token_acc_same_code}{19.1}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_code}{6.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_code}{31.6}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_code}{38.7}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_code}{28.7}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_token_acc_same_code}{22.5}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_same_code}{7.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_same_code}{31.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_same_code}{38.7}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_same_code}{29.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_token_acc_same_code}{23.2}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_same_code}{4.9}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_same_code}{12.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_same_code}{13.8}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_same_code}{12.3}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_token_acc_same_code}{9.1}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_code}{5.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_code}{14.9}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_code}{17.1}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_code}{14.6}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_token_acc_same_code}{11.3}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_same_code}{5.3}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_same_code}{15.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_same_code}{17.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_same_code}{15.1}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_token_acc_same_code}{11.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_code}{14.6}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_code}{44.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_code}{50.4}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_code}{41.2}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_token_acc_same_code}{35.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_same_code}{16.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_same_code}{44.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_same_code}{49.8}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_same_code}{41.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_token_acc_same_code}{34.5}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_same_code}{16.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_same_code}{44.1}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_same_code}{50.2}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_same_code}{41.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_token_acc_same_code}{34.9}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_code}{35.0}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_code}{51.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_code}{53.4}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_code}{51.6}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_token_acc_same_code}{47.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_same_code}{47.4}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_same_code}{60.4}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_same_code}{61.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_same_code}{60.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_token_acc_same_code}{56.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_same_code}{39.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_same_code}{54.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_same_code}{55.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_same_code}{54.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_token_acc_same_code}{49.8}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_same_code}{10.9}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_same_code}{37.0}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_same_code}{42.9}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_same_code}{34.9}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_token_acc_same_code}{28.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_same_code}{14.1}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_same_code}{40.1}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_same_code}{46.4}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_same_code}{37.7}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_token_acc_same_code}{31.1}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_same_code}{14.2}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_same_code}{39.8}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_same_code}{45.7}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_same_code}{37.6}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_token_acc_same_code}{31.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_same_code}{36.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_same_code}{46.8}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_same_code}{48.2}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_same_code}{46.6}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_token_acc_same_code}{43.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_same_code}{43.4}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_same_code}{52.5}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_same_code}{53.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_same_code}{52.2}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_token_acc_same_code}{48.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_same_code}{43.6}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_same_code}{52.5}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_same_code}{53.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_same_code}{52.2}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_token_acc_same_code}{49.2}


==> tables/MN_nd_same_code/table-results-MN_same_code.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_same_code}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_code}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_same_code}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_code}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_same_code}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_code}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_same_code}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_same_code}}
 & $^{\alpha}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_code}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_same_code}
 & $^{\alpha}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_same_code}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-MN_same_code}}
\caption{\UseMacro{TC-results-MN_same_code}}
\end{table}


==> tables/MN_nd_same_code/table-results-aux-MN_same_code.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_p_same_code}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_same_code}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_p_same_code}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_same_code}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_p_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_p_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_r_same_code}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_same_code}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_r_same_code}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_same_code}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_r_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_r_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_f_same_code}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_same_code}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_f_same_code}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_same_code}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_f_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_f_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_same_code}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_same_code}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_exact_match_same_code}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_same_code}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_same_code}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_exact_match_same_code}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_same_code}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_exact_match_same_code}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_same_code}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_exact_match_same_code}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_same_code}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-MN_same_code}}
\caption{\UseMacro{TC-results-aux-MN_same_code}}
\end{table}


==> tables/MN_nd_same_nl/numbers-results-MN.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_same_nl}{0.8}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_same_nl}{26.5}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_same_nl}{36.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_same_nl}{22.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_token_acc_same_nl}{16.5}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_nl}{0.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_nl}{31.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_nl}{42.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_nl}{27.1}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_token_acc_same_nl}{21.0}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_same_nl}{1.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_same_nl}{28.8}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_same_nl}{37.8}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_same_nl}{24.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_token_acc_same_nl}{19.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_same_nl}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_same_nl}{8.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_same_nl}{10.3}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_same_nl}{7.2}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_token_acc_same_nl}{4.7}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_nl}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_nl}{12.9}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_nl}{16.8}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_nl}{11.5}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_token_acc_same_nl}{8.7}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_same_nl}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_same_nl}{10.8}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_same_nl}{13.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_same_nl}{10.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_token_acc_same_nl}{7.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_nl}{2.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_nl}{39.9}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_nl}{50.1}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_nl}{34.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_token_acc_same_nl}{28.1}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_same_nl}{0.9}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_same_nl}{33.3}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_same_nl}{43.9}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_same_nl}{28.3}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_token_acc_same_nl}{20.8}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_same_nl}{2.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_same_nl}{37.8}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_same_nl}{48.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_same_nl}{32.9}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_token_acc_same_nl}{25.3}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_nl}{0.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_nl}{28.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_nl}{31.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_nl}{26.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_token_acc_same_nl}{22.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_same_nl}{0.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_same_nl}{26.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_same_nl}{29.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_same_nl}{25.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_token_acc_same_nl}{18.4}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_same_nl}{0.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_same_nl}{27.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_same_nl}{30.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_same_nl}{26.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_token_acc_same_nl}{20.2}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_same_nl}{2.1}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_same_nl}{29.4}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_same_nl}{39.1}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_same_nl}{24.9}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_token_acc_same_nl}{19.2}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_same_nl}{1.4}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_same_nl}{30.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_same_nl}{40.5}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_same_nl}{25.5}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_token_acc_same_nl}{18.9}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_same_nl}{1.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_same_nl}{30.4}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_same_nl}{40.8}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_same_nl}{25.8}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_token_acc_same_nl}{18.7}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_same_nl}{0.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_same_nl}{13.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_same_nl}{16.4}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_same_nl}{12.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_token_acc_same_nl}{9.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_same_nl}{0.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_same_nl}{14.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_same_nl}{17.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_same_nl}{13.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_token_acc_same_nl}{9.4}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_same_nl}{0.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_same_nl}{13.8}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_same_nl}{17.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_same_nl}{12.6}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_token_acc_same_nl}{8.8}


==> tables/MN_nd_same_nl/table-results-MN_same_nl.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_same_nl}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & $^{\alpha}$\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_same_nl}
 & $^{\beta}$\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_nl}}
 & $^{\alpha}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_same_nl}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_same_nl}}
 & $^{\beta}$\textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_same_nl}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & $^{\gamma}$\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_nl}
 & $^{\gamma}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_same_nl}
 & $^{\delta}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_same_nl}
 & $^{\delta}$\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_same_nl}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_same_nl}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_same_nl}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_same_nl}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-MN_same_nl}}
\caption{\UseMacro{TC-results-MN_same_nl}}
\end{table}


==> tables/MN_nd_same_nl/table-results-aux-MN_same_nl.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_p_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_p_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_p_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_p_same_nl}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_same_nl}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_p_same_nl}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_same_nl}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_p_same_nl}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_r_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_r_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_r_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_r_same_nl}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_same_nl}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_r_same_nl}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_same_nl}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_r_same_nl}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_f_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_f_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_f_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_f_same_nl}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_same_nl}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_f_same_nl}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_same_nl}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_f_same_nl}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_same_nl}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_exact_match_same_nl}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_exact_match_same_nl}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_exact_match_same_nl}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_same_nl}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_exact_match_same_nl}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_same_nl}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_exact_match_same_nl}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_same_nl}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_exact_match_same_nl}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_same_nl}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-MN_same_nl}}
\caption{\UseMacro{TC-results-aux-MN_same_nl}}
\end{table}


==> tables/MN_nd_sim_90/numbers-results-MN.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_sim_90}{0.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_sim_90}{26.1}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_sim_90}{35.7}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_sim_90}{21.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_token_acc_sim_90}{15.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_sim_90}{1.0}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_sim_90}{30.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_sim_90}{40.3}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_sim_90}{25.9}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_token_acc_sim_90}{20.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_sim_90}{1.1}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_sim_90}{28.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_sim_90}{37.2}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_sim_90}{24.4}
\DefMacro{result-MN_CP_Code2SeqICLR19_test_standard_token_acc_sim_90}{18.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_sim_90}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_sim_90}{8.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_sim_90}{10.3}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_sim_90}{7.1}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_token_acc_sim_90}{4.5}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_sim_90}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_sim_90}{11.7}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_sim_90}{15.2}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_sim_90}{10.5}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_token_acc_sim_90}{7.9}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_sim_90}{0.0}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_sim_90}{10.4}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_sim_90}{13.1}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_sim_90}{9.7}
\DefMacro{result-MN_CP_Code2VecPOPL19_test_standard_token_acc_sim_90}{6.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_sim_90}{2.5}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_sim_90}{37.1}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_sim_90}{47.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_sim_90}{32.2}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_token_acc_sim_90}{25.6}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_sim_90}{1.0}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_sim_90}{31.3}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_sim_90}{41.3}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_sim_90}{26.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_token_acc_sim_90}{19.4}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_sim_90}{2.7}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_sim_90}{35.4}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_sim_90}{44.8}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_sim_90}{30.9}
\DefMacro{result-MN_MP_Code2SeqICLR19_test_standard_token_acc_sim_90}{23.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_sim_90}{0.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_sim_90}{23.3}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_sim_90}{26.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_sim_90}{22.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_token_acc_sim_90}{17.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_sim_90}{0.6}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_sim_90}{23.0}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_sim_90}{26.2}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_sim_90}{21.7}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_token_acc_sim_90}{15.5}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_sim_90}{0.1}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_sim_90}{23.6}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_sim_90}{26.8}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_sim_90}{22.6}
\DefMacro{result-MN_MP_Code2VecPOPL19_test_standard_token_acc_sim_90}{17.2}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_sim_90}{2.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_sim_90}{28.5}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_sim_90}{38.0}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_sim_90}{24.2}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_token_acc_sim_90}{18.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_sim_90}{1.7}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_sim_90}{29.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_sim_90}{39.4}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_sim_90}{24.7}
\DefMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_token_acc_sim_90}{18.0}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_sim_90}{1.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_sim_90}{29.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_sim_90}{39.3}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_sim_90}{25.0}
\DefMacro{result-MN_T_Code2SeqICLR19_test_standard_token_acc_sim_90}{17.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_sim_90}{0.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_sim_90}{12.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_sim_90}{14.8}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_sim_90}{10.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_token_acc_sim_90}{7.9}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_sim_90}{0.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_sim_90}{12.5}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_sim_90}{15.2}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_sim_90}{11.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_token_acc_sim_90}{8.1}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_sim_90}{0.0}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_sim_90}{12.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_sim_90}{15.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_sim_90}{11.3}
\DefMacro{result-MN_T_Code2VecPOPL19_test_standard_token_acc_sim_90}{7.8}


==> tables/MN_nd_sim_90/table-results-MN_sim_90.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p_sim_90}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r_sim_90}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f_sim_90}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & $^{\alpha}$\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match_sim_90}
 & $^{\alpha}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match_sim_90}
 & $^{\beta}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match_sim_90}
 & $^{\beta}$\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match_sim_90}}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match_sim_90}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match_sim_90}}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match_sim_90}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-MN_sim_90}}
\caption{\UseMacro{TC-results-MN_sim_90}}
\end{table}


==> tables/MN_nd_sim_90/table-results-aux-MN_sim_90.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_p_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_p_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_p_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_p_sim_90}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p_sim_90}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_p_sim_90}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p_sim_90}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_p_sim_90}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_r_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_r_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_r_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_r_sim_90}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r_sim_90}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_r_sim_90}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r_sim_90}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_r_sim_90}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_f_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_f_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_f_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_f_sim_90}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f_sim_90}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_f_sim_90}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f_sim_90}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_f_sim_90}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f_sim_90}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_val_exact_match_sim_90}
 & \UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_exact_match_sim_90}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_val_exact_match_sim_90}
 & \UseMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match_sim_90}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_exact_match_sim_90}
 & \textbf{\UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match_sim_90}}
 & \UseMacro{result-MN_CP_Code2SeqICLR19_val_exact_match_sim_90}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match_sim_90}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_exact_match_sim_90}
 & \textbf{\UseMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match_sim_90}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-MN_sim_90}}
\caption{\UseMacro{TC-results-aux-MN_sim_90}}
\end{table}


==> tables/numbers-time-wise-dataset-metrics.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{2013_Jan_1-delta}{N/A}
\DefMacro{2013_Jan_1-num-methods}{11183}
\DefMacro{2013_Jan_1-num-projs}{6}
\DefMacro{2014_Jan_1-delta}{740}
\DefMacro{2014_Jan_1-num-methods}{11923}
\DefMacro{2014_Jan_1-num-projs}{10}
\DefMacro{2015_Jan_1-delta}{854}
\DefMacro{2015_Jan_1-num-methods}{12777}
\DefMacro{2015_Jan_1-num-projs}{10}
\DefMacro{2016_Jan_1-delta}{2312}
\DefMacro{2016_Jan_1-num-methods}{15089}
\DefMacro{2016_Jan_1-num-projs}{10}
\DefMacro{2017_Jan_1-delta}{2747}
\DefMacro{2017_Jan_1-num-methods}{17836}
\DefMacro{2017_Jan_1-num-projs}{10}
\DefMacro{2018_Jan_1-delta}{9310}
\DefMacro{2018_Jan_1-num-methods}{27146}
\DefMacro{2018_Jan_1-num-projs}{10}
\DefMacro{2019_Jan_1-delta}{2417}
\DefMacro{2019_Jan_1-num-methods}{29563}
\DefMacro{2019_Jan_1-num-projs}{10}
\DefMacro{2020_Jan_1-delta}{604}
\DefMacro{2020_Jan_1-num-methods}{30167}
\DefMacro{2020_Jan_1-num-projs}{10}


==> tables/table-CG-dataset-metrics-main.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}
\begin{small}
\begin{center}
\caption{\TCDatasetMetricsMainCG}
\begin{tabular}{ l@{\hspace{2pt}}|@{\hspace{2pt}}c@{\hspace{2pt}} | r r r}
\toprule
\multicolumn{2}{c|}{} & & & \\
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \multirow{-2}{*}{\UseMacro{TH-ds-all}} & \multirow{-2}{*}{\UseMacro{TH-ds-2020}} & \multirow{-2}{*}{\UseMacro{TH-ds-2019-2020}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-project}}
 & \UseMacro{ds-CG-num-proj}
 & \UseMacro{ds-CG-num-proj}
 & \UseMacro{ds-CG-num-proj}
\\
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{raw-ds-CG-num-data_all}
 & \UseMacro{ds-CG-num-data_2020}
 & \UseMacro{ds-CG-num-data_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-method-avg}
 & \UseMacro{raw-ds-CG-len-meth-AVG_all}
 & \UseMacro{ds-CG-len-meth-AVG_2020}
 & \UseMacro{ds-CG-len-meth-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-method-mode}
 & \UseMacro{raw-ds-CG-len-meth-MODE_all}
 & \UseMacro{ds-CG-len-meth-MODE_2020}
 & \UseMacro{ds-CG-len-meth-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-method-median}
 & \UseMacro{raw-ds-CG-len-meth-MEDIAN_all}
 & \UseMacro{ds-CG-len-meth-MEDIAN_2020}
 & \UseMacro{ds-CG-len-meth-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-method-le100}
 & \UseMacro{raw-ds-CG-len-meth-le-100_all}
 & \UseMacro{ds-CG-len-meth-le-100_2020}
 & \UseMacro{ds-CG-len-meth-le-100_2019-2020}
\\
& \UseMacro{TH-ds-len-method-le150}
 & \UseMacro{raw-ds-CG-len-meth-le-150_all}
 & \UseMacro{ds-CG-len-meth-le-150_2020}
 & \UseMacro{ds-CG-len-meth-le-150_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-method}} & \UseMacro{TH-ds-len-method-le200}
 & \UseMacro{raw-ds-CG-len-meth-le-200_all}
 & \UseMacro{ds-CG-len-meth-le-200_2020}
 & \UseMacro{ds-CG-len-meth-le-200_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{raw-ds-CG-len-com-AVG_all}
 & \UseMacro{ds-CG-len-com-AVG_2020}
 & \UseMacro{ds-CG-len-com-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-mode}
 & \UseMacro{raw-ds-CG-len-com-MODE_all}
 & \UseMacro{ds-CG-len-com-MODE_2020}
 & \UseMacro{ds-CG-len-com-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-median}
 & \UseMacro{raw-ds-CG-len-com-MEDIAN_all}
 & \UseMacro{ds-CG-len-com-MEDIAN_2020}
 & \UseMacro{ds-CG-len-com-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{raw-ds-CG-len-com-le-20_all}
 & \UseMacro{ds-CG-len-com-le-20_2020}
 & \UseMacro{ds-CG-len-com-le-20_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{raw-ds-CG-len-com-le-30_all}
 & \UseMacro{ds-CG-len-com-le-30_2020}
 & \UseMacro{ds-CG-len-com-le-30_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{raw-ds-CG-len-com-le-50_all}
 & \UseMacro{ds-CG-len-com-le-50_2020}
 & \UseMacro{ds-CG-len-com-le-50_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{raw-ds-CG-len-name-AVG_all}
 & \UseMacro{ds-CG-len-name-AVG_2020}
 & \UseMacro{ds-CG-len-name-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-name-mode}
 & \UseMacro{raw-ds-CG-len-name-MODE_all}
 & \UseMacro{ds-CG-len-name-MODE_2020}
 & \UseMacro{ds-CG-len-name-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-name-median}
 & \UseMacro{raw-ds-CG-len-name-MEDIAN_all}
 & \UseMacro{ds-CG-len-name-MEDIAN_2020}
 & \UseMacro{ds-CG-len-name-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{raw-ds-CG-len-name-le-3_all}
 & \UseMacro{ds-CG-len-name-le-3_2020}
 & \UseMacro{ds-CG-len-name-le-3_2019-2020}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{raw-ds-CG-len-name-le-5_all}
 & \UseMacro{ds-CG-len-name-le-5_2020}
 & \UseMacro{ds-CG-len-name-le-5_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{raw-ds-CG-len-name-le-6_all}
 & \UseMacro{ds-CG-len-name-le-6_2020}
 & \UseMacro{ds-CG-len-name-le-6_2019-2020}
\\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{\TVDatasetMetricsMainCG}
\end{table}


==> tables/table-CG-dataset-metrics-split.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}
\begin{small}
\begin{center}
\caption{\TCDatasetMetricsSplitCG}
\begin{tabular}{ l@{\hspace{2pt}}|@{\hspace{2pt}}c@{\hspace{2pt}} | rr @{\hspace{5pt}}c@{\hspace{5pt}} rr @{\hspace{5pt}}c@{\hspace{5pt}} rr r}
\toprule
\multicolumn{2}{c|}{} & \multicolumn{2}{c}{\UseMacro{TH-ds-mixedproj}} & & \multicolumn{2}{c}{\UseMacro{TH-ds-crossproj}} & & \multicolumn{2}{c}{\UseMacro{TH-ds-evo}} & \\\cline{3-4}\cline{6-7}\cline{9-10}
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \UseMacro{TH-ds-mixedproj-train} & \UseMacro{TH-ds-mixedproj-val} & & \UseMacro{TH-ds-crossproj-train} & \UseMacro{TH-ds-crossproj-val} & & \UseMacro{TH-ds-evo-train} & \UseMacro{TH-ds-evo-val} & \multirow{-2}{*}{\UseMacro{TH-ds-test}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-project}}
 & \UseMacro{ds-CG-num-proj}
 & \UseMacro{ds-CG-num-proj}
 & 
 & \UseMacro{ds-CG-num-proj_train}
 & \UseMacro{ds-CG-num-proj_val}
 & 
 & \UseMacro{ds-CG-num-proj}
 & \UseMacro{ds-CG-num-proj}
 & \UseMacro{ds-CG-num-proj_test}
\\
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{ds-CG-num-data_mixedproj-2020-train}
 & \UseMacro{ds-CG-num-data_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-num-data_crossproj-2020-train}
 & \UseMacro{ds-CG-num-data_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-num-data_evo-2020-train}
 & \UseMacro{ds-CG-num-data_evo-2020-val}
 & \UseMacro{ds-CG-num-data_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-method-avg}
 & \UseMacro{ds-CG-len-meth-AVG_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-AVG_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-AVG_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-AVG_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-mode}
 & \UseMacro{ds-CG-len-meth-MODE_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-MODE_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-MODE_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-MODE_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-median}
 & \UseMacro{ds-CG-len-meth-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-MEDIAN_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-MEDIAN_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-le100}
 & \UseMacro{ds-CG-len-meth-le-100_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-100_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-100_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-100_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-100_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-le-100_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-le-100_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-le150}
 & \UseMacro{ds-CG-len-meth-le-150_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-150_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-150_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-150_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-150_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-le-150_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-le-150_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-method}} & \UseMacro{TH-ds-len-method-le200}
 & \UseMacro{ds-CG-len-meth-le-200_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-200_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-200_crossproj-2020-train}
 & \UseMacro{ds-CG-len-meth-le-200_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-meth-le-200_evo-2020-train}
 & \UseMacro{ds-CG-len-meth-le-200_evo-2020-val}
 & \UseMacro{ds-CG-len-meth-le-200_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{ds-CG-len-com-AVG_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-AVG_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-AVG_evo-2020-train}
 & \UseMacro{ds-CG-len-com-AVG_evo-2020-val}
 & \UseMacro{ds-CG-len-com-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-mode}
 & \UseMacro{ds-CG-len-com-MODE_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-MODE_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-MODE_evo-2020-train}
 & \UseMacro{ds-CG-len-com-MODE_evo-2020-val}
 & \UseMacro{ds-CG-len-com-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-median}
 & \UseMacro{ds-CG-len-com-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-MEDIAN_evo-2020-train}
 & \UseMacro{ds-CG-len-com-MEDIAN_evo-2020-val}
 & \UseMacro{ds-CG-len-com-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{ds-CG-len-com-le-20_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-20_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-20_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-20_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-20_evo-2020-train}
 & \UseMacro{ds-CG-len-com-le-20_evo-2020-val}
 & \UseMacro{ds-CG-len-com-le-20_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{ds-CG-len-com-le-30_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-30_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-30_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-30_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-30_evo-2020-train}
 & \UseMacro{ds-CG-len-com-le-30_evo-2020-val}
 & \UseMacro{ds-CG-len-com-le-30_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{ds-CG-len-com-le-50_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-50_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-50_crossproj-2020-train}
 & \UseMacro{ds-CG-len-com-le-50_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-com-le-50_evo-2020-train}
 & \UseMacro{ds-CG-len-com-le-50_evo-2020-val}
 & \UseMacro{ds-CG-len-com-le-50_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{ds-CG-len-name-AVG_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-AVG_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-AVG_evo-2020-train}
 & \UseMacro{ds-CG-len-name-AVG_evo-2020-val}
 & \UseMacro{ds-CG-len-name-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-mode}
 & \UseMacro{ds-CG-len-name-MODE_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-MODE_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-MODE_evo-2020-train}
 & \UseMacro{ds-CG-len-name-MODE_evo-2020-val}
 & \UseMacro{ds-CG-len-name-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-median}
 & \UseMacro{ds-CG-len-name-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-MEDIAN_evo-2020-train}
 & \UseMacro{ds-CG-len-name-MEDIAN_evo-2020-val}
 & \UseMacro{ds-CG-len-name-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{ds-CG-len-name-le-3_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-3_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-3_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-3_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-3_evo-2020-train}
 & \UseMacro{ds-CG-len-name-le-3_evo-2020-val}
 & \UseMacro{ds-CG-len-name-le-3_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{ds-CG-len-name-le-5_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-5_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-5_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-5_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-5_evo-2020-train}
 & \UseMacro{ds-CG-len-name-le-5_evo-2020-val}
 & \UseMacro{ds-CG-len-name-le-5_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{ds-CG-len-name-le-6_mixedproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-6_mixedproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-6_crossproj-2020-train}
 & \UseMacro{ds-CG-len-name-le-6_crossproj-2020-val}
 & 
 & \UseMacro{ds-CG-len-name-le-6_evo-2020-train}
 & \UseMacro{ds-CG-len-name-le-6_evo-2020-val}
 & \UseMacro{ds-CG-len-name-le-6_2020-test_common}
\\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{\TVDatasetMetricsSplitCG}
\end{table*}


==> tables/table-MN-dataset-metrics-main.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}
\begin{small}
\begin{center}
\caption{\TCDatasetMetricsMainMN}
\begin{tabular}{ l@{\hspace{2pt}}|@{\hspace{2pt}}c@{\hspace{2pt}} | r r r}
\toprule
\multicolumn{2}{c|}{} & & & \\
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \multirow{-2}{*}{\UseMacro{TH-ds-all}} & \multirow{-2}{*}{\UseMacro{TH-ds-2020}} & \multirow{-2}{*}{\UseMacro{TH-ds-2019-2020}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-project}}
 & \UseMacro{ds-MN-num-proj}
 & \UseMacro{ds-MN-num-proj}
 & \UseMacro{ds-MN-num-proj}
\\
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{raw-ds-MN-num-data_all}
 & \UseMacro{ds-MN-num-data_2020}
 & \UseMacro{ds-MN-num-data_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-method-avg}
 & \UseMacro{raw-ds-MN-len-meth-AVG_all}
 & \UseMacro{ds-MN-len-meth-AVG_2020}
 & \UseMacro{ds-MN-len-meth-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-method-mode}
 & \UseMacro{raw-ds-MN-len-meth-MODE_all}
 & \UseMacro{ds-MN-len-meth-MODE_2020}
 & \UseMacro{ds-MN-len-meth-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-method-median}
 & \UseMacro{raw-ds-MN-len-meth-MEDIAN_all}
 & \UseMacro{ds-MN-len-meth-MEDIAN_2020}
 & \UseMacro{ds-MN-len-meth-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-method-le100}
 & \UseMacro{raw-ds-MN-len-meth-le-100_all}
 & \UseMacro{ds-MN-len-meth-le-100_2020}
 & \UseMacro{ds-MN-len-meth-le-100_2019-2020}
\\
& \UseMacro{TH-ds-len-method-le150}
 & \UseMacro{raw-ds-MN-len-meth-le-150_all}
 & \UseMacro{ds-MN-len-meth-le-150_2020}
 & \UseMacro{ds-MN-len-meth-le-150_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-method}} & \UseMacro{TH-ds-len-method-le200}
 & \UseMacro{raw-ds-MN-len-meth-le-200_all}
 & \UseMacro{ds-MN-len-meth-le-200_2020}
 & \UseMacro{ds-MN-len-meth-le-200_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{raw-ds-MN-len-com-AVG_all}
 & \UseMacro{ds-MN-len-com-AVG_2020}
 & \UseMacro{ds-MN-len-com-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-mode}
 & \UseMacro{raw-ds-MN-len-com-MODE_all}
 & \UseMacro{ds-MN-len-com-MODE_2020}
 & \UseMacro{ds-MN-len-com-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-median}
 & \UseMacro{raw-ds-MN-len-com-MEDIAN_all}
 & \UseMacro{ds-MN-len-com-MEDIAN_2020}
 & \UseMacro{ds-MN-len-com-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{raw-ds-MN-len-com-le-20_all}
 & \UseMacro{ds-MN-len-com-le-20_2020}
 & \UseMacro{ds-MN-len-com-le-20_2019-2020}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{raw-ds-MN-len-com-le-30_all}
 & \UseMacro{ds-MN-len-com-le-30_2020}
 & \UseMacro{ds-MN-len-com-le-30_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{raw-ds-MN-len-com-le-50_all}
 & \UseMacro{ds-MN-len-com-le-50_2020}
 & \UseMacro{ds-MN-len-com-le-50_2019-2020}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{raw-ds-MN-len-name-AVG_all}
 & \UseMacro{ds-MN-len-name-AVG_2020}
 & \UseMacro{ds-MN-len-name-AVG_2019-2020}
\\
& \UseMacro{TH-ds-len-name-mode}
 & \UseMacro{raw-ds-MN-len-name-MODE_all}
 & \UseMacro{ds-MN-len-name-MODE_2020}
 & \UseMacro{ds-MN-len-name-MODE_2019-2020}
\\
& \UseMacro{TH-ds-len-name-median}
 & \UseMacro{raw-ds-MN-len-name-MEDIAN_all}
 & \UseMacro{ds-MN-len-name-MEDIAN_2020}
 & \UseMacro{ds-MN-len-name-MEDIAN_2019-2020}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{raw-ds-MN-len-name-le-3_all}
 & \UseMacro{ds-MN-len-name-le-3_2020}
 & \UseMacro{ds-MN-len-name-le-3_2019-2020}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{raw-ds-MN-len-name-le-5_all}
 & \UseMacro{ds-MN-len-name-le-5_2020}
 & \UseMacro{ds-MN-len-name-le-5_2019-2020}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{raw-ds-MN-len-name-le-6_all}
 & \UseMacro{ds-MN-len-name-le-6_2020}
 & \UseMacro{ds-MN-len-name-le-6_2019-2020}
\\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{\TVDatasetMetricsMainMN}
\end{table}


==> tables/table-MN-dataset-metrics-split.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}
\begin{small}
\begin{center}
\caption{\TCDatasetMetricsSplitMN}
\begin{tabular}{ l@{\hspace{2pt}}|@{\hspace{2pt}}c@{\hspace{2pt}} | rr @{\hspace{5pt}}c@{\hspace{5pt}} rr @{\hspace{5pt}}c@{\hspace{5pt}} rr r}
\toprule
\multicolumn{2}{c|}{} & \multicolumn{2}{c}{\UseMacro{TH-ds-mixedproj}} & & \multicolumn{2}{c}{\UseMacro{TH-ds-crossproj}} & & \multicolumn{2}{c}{\UseMacro{TH-ds-evo}} & \\\cline{3-4}\cline{6-7}\cline{9-10}
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \UseMacro{TH-ds-mixedproj-train} & \UseMacro{TH-ds-mixedproj-val} & & \UseMacro{TH-ds-crossproj-train} & \UseMacro{TH-ds-crossproj-val} & & \UseMacro{TH-ds-evo-train} & \UseMacro{TH-ds-evo-val} & \multirow{-2}{*}{\UseMacro{TH-ds-test}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-project}}
 & \UseMacro{ds-MN-num-proj}
 & \UseMacro{ds-MN-num-proj}
 & 
 & \UseMacro{ds-MN-num-proj_train}
 & \UseMacro{ds-MN-num-proj_val}
 & 
 & \UseMacro{ds-MN-num-proj}
 & \UseMacro{ds-MN-num-proj}
 & \UseMacro{ds-MN-num-proj_test}
\\
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{ds-MN-num-data_mixedproj-2020-train}
 & \UseMacro{ds-MN-num-data_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-num-data_crossproj-2020-train}
 & \UseMacro{ds-MN-num-data_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-num-data_evo-2020-train}
 & \UseMacro{ds-MN-num-data_evo-2020-val}
 & \UseMacro{ds-MN-num-data_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-method-avg}
 & \UseMacro{ds-MN-len-meth-AVG_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-AVG_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-AVG_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-AVG_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-mode}
 & \UseMacro{ds-MN-len-meth-MODE_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-MODE_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-MODE_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-MODE_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-median}
 & \UseMacro{ds-MN-len-meth-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-MEDIAN_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-MEDIAN_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-le100}
 & \UseMacro{ds-MN-len-meth-le-100_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-100_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-100_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-100_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-100_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-le-100_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-le-100_2020-test_common}
\\
& \UseMacro{TH-ds-len-method-le150}
 & \UseMacro{ds-MN-len-meth-le-150_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-150_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-150_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-150_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-150_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-le-150_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-le-150_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-method}} & \UseMacro{TH-ds-len-method-le200}
 & \UseMacro{ds-MN-len-meth-le-200_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-200_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-200_crossproj-2020-train}
 & \UseMacro{ds-MN-len-meth-le-200_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-meth-le-200_evo-2020-train}
 & \UseMacro{ds-MN-len-meth-le-200_evo-2020-val}
 & \UseMacro{ds-MN-len-meth-le-200_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{ds-MN-len-com-AVG_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-AVG_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-AVG_evo-2020-train}
 & \UseMacro{ds-MN-len-com-AVG_evo-2020-val}
 & \UseMacro{ds-MN-len-com-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-mode}
 & \UseMacro{ds-MN-len-com-MODE_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-MODE_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-MODE_evo-2020-train}
 & \UseMacro{ds-MN-len-com-MODE_evo-2020-val}
 & \UseMacro{ds-MN-len-com-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-median}
 & \UseMacro{ds-MN-len-com-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-MEDIAN_evo-2020-train}
 & \UseMacro{ds-MN-len-com-MEDIAN_evo-2020-val}
 & \UseMacro{ds-MN-len-com-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{ds-MN-len-com-le-20_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-20_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-20_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-20_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-20_evo-2020-train}
 & \UseMacro{ds-MN-len-com-le-20_evo-2020-val}
 & \UseMacro{ds-MN-len-com-le-20_2020-test_common}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{ds-MN-len-com-le-30_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-30_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-30_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-30_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-30_evo-2020-train}
 & \UseMacro{ds-MN-len-com-le-30_evo-2020-val}
 & \UseMacro{ds-MN-len-com-le-30_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{ds-MN-len-com-le-50_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-50_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-50_crossproj-2020-train}
 & \UseMacro{ds-MN-len-com-le-50_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-com-le-50_evo-2020-train}
 & \UseMacro{ds-MN-len-com-le-50_evo-2020-val}
 & \UseMacro{ds-MN-len-com-le-50_2020-test_common}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{ds-MN-len-name-AVG_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-AVG_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-AVG_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-AVG_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-AVG_evo-2020-train}
 & \UseMacro{ds-MN-len-name-AVG_evo-2020-val}
 & \UseMacro{ds-MN-len-name-AVG_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-mode}
 & \UseMacro{ds-MN-len-name-MODE_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-MODE_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-MODE_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-MODE_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-MODE_evo-2020-train}
 & \UseMacro{ds-MN-len-name-MODE_evo-2020-val}
 & \UseMacro{ds-MN-len-name-MODE_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-median}
 & \UseMacro{ds-MN-len-name-MEDIAN_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-MEDIAN_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-MEDIAN_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-MEDIAN_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-MEDIAN_evo-2020-train}
 & \UseMacro{ds-MN-len-name-MEDIAN_evo-2020-val}
 & \UseMacro{ds-MN-len-name-MEDIAN_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{ds-MN-len-name-le-3_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-3_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-3_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-3_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-3_evo-2020-train}
 & \UseMacro{ds-MN-len-name-le-3_evo-2020-val}
 & \UseMacro{ds-MN-len-name-le-3_2020-test_common}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{ds-MN-len-name-le-5_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-5_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-5_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-5_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-5_evo-2020-train}
 & \UseMacro{ds-MN-len-name-le-5_evo-2020-val}
 & \UseMacro{ds-MN-len-name-le-5_2020-test_common}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{ds-MN-len-name-le-6_mixedproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-6_mixedproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-6_crossproj-2020-train}
 & \UseMacro{ds-MN-len-name-le-6_crossproj-2020-val}
 & 
 & \UseMacro{ds-MN-len-name-le-6_evo-2020-train}
 & \UseMacro{ds-MN-len-name-le-6_evo-2020-val}
 & \UseMacro{ds-MN-len-name-le-6_2020-test_common}
\\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{\TVDatasetMetricsSplitMN}
\end{table*}


==> tables/table-dataset-metrics-CG.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{ l@{\hspace{2pt}}c@{\hspace{2pt}} | r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r }
\toprule
\multicolumn{2}{c|}{} & \multicolumn{3}{c}{\UseMacro{TH-ds-MP}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-CP}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-T}} & & \UseMacro{TH-ds-MP-CP} & \UseMacro{TH-ds-MP-T} & \UseMacro{TH-ds-CP-T} \\\cline{3-5}\cline{7-9}\cline{11-13}\cline{15-17}
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \multicolumn{3}{c}{\UseMacro{TH-ds-test_common}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{ds-CG-train-MP_num-data}
 & \UseMacro{ds-CG-val-MP_num-data}
 & \UseMacro{ds-CG-test_standard-MP_num-data}
 & 
 & \UseMacro{ds-CG-train-CP_num-data}
 & \UseMacro{ds-CG-val-CP_num-data}
 & \UseMacro{ds-CG-test_standard-CP_num-data}
 & 
 & \UseMacro{ds-CG-train-T_num-data}
 & \UseMacro{ds-CG-val-T_num-data}
 & \UseMacro{ds-CG-test_standard-T_num-data}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_num-data}
 & \UseMacro{ds-CG-test_common-MP-T_num-data}
 & \UseMacro{ds-CG-test_common-CP-T_num-data}
\\
\midrule
& \UseMacro{TH-ds-len-code-avg}
 & \UseMacro{ds-CG-train-MP_len-code-AVG}
 & \UseMacro{ds-CG-val-MP_len-code-AVG}
 & \UseMacro{ds-CG-test_standard-MP_len-code-AVG}
 & 
 & \UseMacro{ds-CG-train-CP_len-code-AVG}
 & \UseMacro{ds-CG-val-CP_len-code-AVG}
 & \UseMacro{ds-CG-test_standard-CP_len-code-AVG}
 & 
 & \UseMacro{ds-CG-train-T_len-code-AVG}
 & \UseMacro{ds-CG-val-T_len-code-AVG}
 & \UseMacro{ds-CG-test_standard-T_len-code-AVG}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-code-AVG}
 & \UseMacro{ds-CG-test_common-MP-T_len-code-AVG}
 & \UseMacro{ds-CG-test_common-CP-T_len-code-AVG}
\\
& \UseMacro{TH-ds-len-code-le100}
 & \UseMacro{ds-CG-train-MP_len-code-le-100}
 & \UseMacro{ds-CG-val-MP_len-code-le-100}
 & \UseMacro{ds-CG-test_standard-MP_len-code-le-100}
 & 
 & \UseMacro{ds-CG-train-CP_len-code-le-100}
 & \UseMacro{ds-CG-val-CP_len-code-le-100}
 & \UseMacro{ds-CG-test_standard-CP_len-code-le-100}
 & 
 & \UseMacro{ds-CG-train-T_len-code-le-100}
 & \UseMacro{ds-CG-val-T_len-code-le-100}
 & \UseMacro{ds-CG-test_standard-T_len-code-le-100}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-code-le-100}
 & \UseMacro{ds-CG-test_common-MP-T_len-code-le-100}
 & \UseMacro{ds-CG-test_common-CP-T_len-code-le-100}
\\
& \UseMacro{TH-ds-len-code-le150}
 & \UseMacro{ds-CG-train-MP_len-code-le-150}
 & \UseMacro{ds-CG-val-MP_len-code-le-150}
 & \UseMacro{ds-CG-test_standard-MP_len-code-le-150}
 & 
 & \UseMacro{ds-CG-train-CP_len-code-le-150}
 & \UseMacro{ds-CG-val-CP_len-code-le-150}
 & \UseMacro{ds-CG-test_standard-CP_len-code-le-150}
 & 
 & \UseMacro{ds-CG-train-T_len-code-le-150}
 & \UseMacro{ds-CG-val-T_len-code-le-150}
 & \UseMacro{ds-CG-test_standard-T_len-code-le-150}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-code-le-150}
 & \UseMacro{ds-CG-test_common-MP-T_len-code-le-150}
 & \UseMacro{ds-CG-test_common-CP-T_len-code-le-150}
\\
\multirow{-4}{*}{\UseMacro{TH-ds-len-code}} & \UseMacro{TH-ds-len-code-le200}
 & \UseMacro{ds-CG-train-MP_len-code-le-200}
 & \UseMacro{ds-CG-val-MP_len-code-le-200}
 & \UseMacro{ds-CG-test_standard-MP_len-code-le-200}
 & 
 & \UseMacro{ds-CG-train-CP_len-code-le-200}
 & \UseMacro{ds-CG-val-CP_len-code-le-200}
 & \UseMacro{ds-CG-test_standard-CP_len-code-le-200}
 & 
 & \UseMacro{ds-CG-train-T_len-code-le-200}
 & \UseMacro{ds-CG-val-T_len-code-le-200}
 & \UseMacro{ds-CG-test_standard-T_len-code-le-200}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-code-le-200}
 & \UseMacro{ds-CG-test_common-MP-T_len-code-le-200}
 & \UseMacro{ds-CG-test_common-CP-T_len-code-le-200}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{ds-CG-train-MP_len-comment-AVG}
 & \UseMacro{ds-CG-val-MP_len-comment-AVG}
 & \UseMacro{ds-CG-test_standard-MP_len-comment-AVG}
 & 
 & \UseMacro{ds-CG-train-CP_len-comment-AVG}
 & \UseMacro{ds-CG-val-CP_len-comment-AVG}
 & \UseMacro{ds-CG-test_standard-CP_len-comment-AVG}
 & 
 & \UseMacro{ds-CG-train-T_len-comment-AVG}
 & \UseMacro{ds-CG-val-T_len-comment-AVG}
 & \UseMacro{ds-CG-test_standard-T_len-comment-AVG}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-comment-AVG}
 & \UseMacro{ds-CG-test_common-MP-T_len-comment-AVG}
 & \UseMacro{ds-CG-test_common-CP-T_len-comment-AVG}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{ds-CG-train-MP_len-comment-le-20}
 & \UseMacro{ds-CG-val-MP_len-comment-le-20}
 & \UseMacro{ds-CG-test_standard-MP_len-comment-le-20}
 & 
 & \UseMacro{ds-CG-train-CP_len-comment-le-20}
 & \UseMacro{ds-CG-val-CP_len-comment-le-20}
 & \UseMacro{ds-CG-test_standard-CP_len-comment-le-20}
 & 
 & \UseMacro{ds-CG-train-T_len-comment-le-20}
 & \UseMacro{ds-CG-val-T_len-comment-le-20}
 & \UseMacro{ds-CG-test_standard-T_len-comment-le-20}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-comment-le-20}
 & \UseMacro{ds-CG-test_common-MP-T_len-comment-le-20}
 & \UseMacro{ds-CG-test_common-CP-T_len-comment-le-20}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{ds-CG-train-MP_len-comment-le-30}
 & \UseMacro{ds-CG-val-MP_len-comment-le-30}
 & \UseMacro{ds-CG-test_standard-MP_len-comment-le-30}
 & 
 & \UseMacro{ds-CG-train-CP_len-comment-le-30}
 & \UseMacro{ds-CG-val-CP_len-comment-le-30}
 & \UseMacro{ds-CG-test_standard-CP_len-comment-le-30}
 & 
 & \UseMacro{ds-CG-train-T_len-comment-le-30}
 & \UseMacro{ds-CG-val-T_len-comment-le-30}
 & \UseMacro{ds-CG-test_standard-T_len-comment-le-30}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-comment-le-30}
 & \UseMacro{ds-CG-test_common-MP-T_len-comment-le-30}
 & \UseMacro{ds-CG-test_common-CP-T_len-comment-le-30}
\\
\multirow{-4}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{ds-CG-train-MP_len-comment-le-50}
 & \UseMacro{ds-CG-val-MP_len-comment-le-50}
 & \UseMacro{ds-CG-test_standard-MP_len-comment-le-50}
 & 
 & \UseMacro{ds-CG-train-CP_len-comment-le-50}
 & \UseMacro{ds-CG-val-CP_len-comment-le-50}
 & \UseMacro{ds-CG-test_standard-CP_len-comment-le-50}
 & 
 & \UseMacro{ds-CG-train-T_len-comment-le-50}
 & \UseMacro{ds-CG-val-T_len-comment-le-50}
 & \UseMacro{ds-CG-test_standard-T_len-comment-le-50}
 & 
 & \UseMacro{ds-CG-test_common-MP-CP_len-comment-le-50}
 & \UseMacro{ds-CG-test_common-MP-T_len-comment-le-50}
 & \UseMacro{ds-CG-test_common-CP-T_len-comment-le-50}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-dataset-metrics-CG}}
\caption{\UseMacro{TC-dataset-metrics-CG}}
\end{table*}


==> tables/table-dataset-metrics-MN.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{ l@{\hspace{2pt}}c@{\hspace{2pt}} | r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r @{\hspace{3pt}}c@{\hspace{3pt}} r@{\hspace{4pt}}r@{\hspace{4pt}}r }
\toprule
\multicolumn{2}{c|}{} & \multicolumn{3}{c}{\UseMacro{TH-ds-MP}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-CP}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-T}} & & \UseMacro{TH-ds-MP-CP} & \UseMacro{TH-ds-MP-T} & \UseMacro{TH-ds-CP-T} \\\cline{3-5}\cline{7-9}\cline{11-13}\cline{15-17}
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \multicolumn{3}{c}{\UseMacro{TH-ds-test_common}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{ds-MN-train-MP_num-data}
 & \UseMacro{ds-MN-val-MP_num-data}
 & \UseMacro{ds-MN-test_standard-MP_num-data}
 & 
 & \UseMacro{ds-MN-train-CP_num-data}
 & \UseMacro{ds-MN-val-CP_num-data}
 & \UseMacro{ds-MN-test_standard-CP_num-data}
 & 
 & \UseMacro{ds-MN-train-T_num-data}
 & \UseMacro{ds-MN-val-T_num-data}
 & \UseMacro{ds-MN-test_standard-T_num-data}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_num-data}
 & \UseMacro{ds-MN-test_common-MP-T_num-data}
 & \UseMacro{ds-MN-test_common-CP-T_num-data}
\\
\midrule
& \UseMacro{TH-ds-len-code-avg}
 & \UseMacro{ds-MN-train-MP_len-code-AVG}
 & \UseMacro{ds-MN-val-MP_len-code-AVG}
 & \UseMacro{ds-MN-test_standard-MP_len-code-AVG}
 & 
 & \UseMacro{ds-MN-train-CP_len-code-AVG}
 & \UseMacro{ds-MN-val-CP_len-code-AVG}
 & \UseMacro{ds-MN-test_standard-CP_len-code-AVG}
 & 
 & \UseMacro{ds-MN-train-T_len-code-AVG}
 & \UseMacro{ds-MN-val-T_len-code-AVG}
 & \UseMacro{ds-MN-test_standard-T_len-code-AVG}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-code-AVG}
 & \UseMacro{ds-MN-test_common-MP-T_len-code-AVG}
 & \UseMacro{ds-MN-test_common-CP-T_len-code-AVG}
\\
& \UseMacro{TH-ds-len-code-le100}
 & \UseMacro{ds-MN-train-MP_len-code-le-100}
 & \UseMacro{ds-MN-val-MP_len-code-le-100}
 & \UseMacro{ds-MN-test_standard-MP_len-code-le-100}
 & 
 & \UseMacro{ds-MN-train-CP_len-code-le-100}
 & \UseMacro{ds-MN-val-CP_len-code-le-100}
 & \UseMacro{ds-MN-test_standard-CP_len-code-le-100}
 & 
 & \UseMacro{ds-MN-train-T_len-code-le-100}
 & \UseMacro{ds-MN-val-T_len-code-le-100}
 & \UseMacro{ds-MN-test_standard-T_len-code-le-100}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-code-le-100}
 & \UseMacro{ds-MN-test_common-MP-T_len-code-le-100}
 & \UseMacro{ds-MN-test_common-CP-T_len-code-le-100}
\\
& \UseMacro{TH-ds-len-code-le150}
 & \UseMacro{ds-MN-train-MP_len-code-le-150}
 & \UseMacro{ds-MN-val-MP_len-code-le-150}
 & \UseMacro{ds-MN-test_standard-MP_len-code-le-150}
 & 
 & \UseMacro{ds-MN-train-CP_len-code-le-150}
 & \UseMacro{ds-MN-val-CP_len-code-le-150}
 & \UseMacro{ds-MN-test_standard-CP_len-code-le-150}
 & 
 & \UseMacro{ds-MN-train-T_len-code-le-150}
 & \UseMacro{ds-MN-val-T_len-code-le-150}
 & \UseMacro{ds-MN-test_standard-T_len-code-le-150}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-code-le-150}
 & \UseMacro{ds-MN-test_common-MP-T_len-code-le-150}
 & \UseMacro{ds-MN-test_common-CP-T_len-code-le-150}
\\
\multirow{-4}{*}{\UseMacro{TH-ds-len-code}} & \UseMacro{TH-ds-len-code-le200}
 & \UseMacro{ds-MN-train-MP_len-code-le-200}
 & \UseMacro{ds-MN-val-MP_len-code-le-200}
 & \UseMacro{ds-MN-test_standard-MP_len-code-le-200}
 & 
 & \UseMacro{ds-MN-train-CP_len-code-le-200}
 & \UseMacro{ds-MN-val-CP_len-code-le-200}
 & \UseMacro{ds-MN-test_standard-CP_len-code-le-200}
 & 
 & \UseMacro{ds-MN-train-T_len-code-le-200}
 & \UseMacro{ds-MN-val-T_len-code-le-200}
 & \UseMacro{ds-MN-test_standard-T_len-code-le-200}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-code-le-200}
 & \UseMacro{ds-MN-test_common-MP-T_len-code-le-200}
 & \UseMacro{ds-MN-test_common-CP-T_len-code-le-200}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{ds-MN-train-MP_len-name-AVG}
 & \UseMacro{ds-MN-val-MP_len-name-AVG}
 & \UseMacro{ds-MN-test_standard-MP_len-name-AVG}
 & 
 & \UseMacro{ds-MN-train-CP_len-name-AVG}
 & \UseMacro{ds-MN-val-CP_len-name-AVG}
 & \UseMacro{ds-MN-test_standard-CP_len-name-AVG}
 & 
 & \UseMacro{ds-MN-train-T_len-name-AVG}
 & \UseMacro{ds-MN-val-T_len-name-AVG}
 & \UseMacro{ds-MN-test_standard-T_len-name-AVG}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-name-AVG}
 & \UseMacro{ds-MN-test_common-MP-T_len-name-AVG}
 & \UseMacro{ds-MN-test_common-CP-T_len-name-AVG}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{ds-MN-train-MP_len-name-le-2}
 & \UseMacro{ds-MN-val-MP_len-name-le-2}
 & \UseMacro{ds-MN-test_standard-MP_len-name-le-2}
 & 
 & \UseMacro{ds-MN-train-CP_len-name-le-2}
 & \UseMacro{ds-MN-val-CP_len-name-le-2}
 & \UseMacro{ds-MN-test_standard-CP_len-name-le-2}
 & 
 & \UseMacro{ds-MN-train-T_len-name-le-2}
 & \UseMacro{ds-MN-val-T_len-name-le-2}
 & \UseMacro{ds-MN-test_standard-T_len-name-le-2}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-name-le-2}
 & \UseMacro{ds-MN-test_common-MP-T_len-name-le-2}
 & \UseMacro{ds-MN-test_common-CP-T_len-name-le-2}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{ds-MN-train-MP_len-name-le-3}
 & \UseMacro{ds-MN-val-MP_len-name-le-3}
 & \UseMacro{ds-MN-test_standard-MP_len-name-le-3}
 & 
 & \UseMacro{ds-MN-train-CP_len-name-le-3}
 & \UseMacro{ds-MN-val-CP_len-name-le-3}
 & \UseMacro{ds-MN-test_standard-CP_len-name-le-3}
 & 
 & \UseMacro{ds-MN-train-T_len-name-le-3}
 & \UseMacro{ds-MN-val-T_len-name-le-3}
 & \UseMacro{ds-MN-test_standard-T_len-name-le-3}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-name-le-3}
 & \UseMacro{ds-MN-test_common-MP-T_len-name-le-3}
 & \UseMacro{ds-MN-test_common-CP-T_len-name-le-3}
\\
\multirow{-4}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{ds-MN-train-MP_len-name-le-6}
 & \UseMacro{ds-MN-val-MP_len-name-le-6}
 & \UseMacro{ds-MN-test_standard-MP_len-name-le-6}
 & 
 & \UseMacro{ds-MN-train-CP_len-name-le-6}
 & \UseMacro{ds-MN-val-CP_len-name-le-6}
 & \UseMacro{ds-MN-test_standard-CP_len-name-le-6}
 & 
 & \UseMacro{ds-MN-train-T_len-name-le-6}
 & \UseMacro{ds-MN-val-T_len-name-le-6}
 & \UseMacro{ds-MN-test_standard-T_len-name-le-6}
 & 
 & \UseMacro{ds-MN-test_common-MP-CP_len-name-le-6}
 & \UseMacro{ds-MN-test_common-MP-T_len-name-le-6}
 & \UseMacro{ds-MN-test_common-CP-T_len-name-le-6}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-dataset-metrics-MN}}
\caption{\UseMacro{TC-dataset-metrics-MN}}
\end{table*}


==> tables/table-dataset-metrics-small.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{ @{\hspace{2pt}} l @{\hspace{2pt}} | @{\hspace{3pt}} c @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{5pt}} r @{\hspace{3pt}}c@{\hspace{3pt}} c @{\hspace{5pt}} r@{\hspace{2pt}} }
\toprule
\textbf{Task} & & \textbf{\ATrain} & \textbf{\AVal} & \textbf{\ATestS} & & & \textbf{\ATestC} \\
\midrule
 & \UseMacro{TH-ds-MP}
 & \UseMacro{ds-CG-train-MP_num-data}
 & \UseMacro{ds-CG-val-MP_num-data}
 & \UseMacro{ds-CG-test_standard-MP_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (CGMP-base) {\phantom{XX}};
 & \UseMacro{TH-ds-MP-CP}
 & \UseMacro{ds-CG-test_common-MP-CP_num-data}
\\
 & \UseMacro{TH-ds-CP}
 & \UseMacro{ds-CG-train-CP_num-data}
 & \UseMacro{ds-CG-val-CP_num-data}
 & \UseMacro{ds-CG-test_standard-CP_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (CGCP-base) {\phantom{XX}};
 & \UseMacro{TH-ds-MP-T}
 & \UseMacro{ds-CG-test_common-MP-T_num-data}
\\
\multirow{-3.5}{*}{\rotatebox[origin=c]{90}{\UseMacro{TaskM_CG}}}
 & \UseMacro{TH-ds-T}
 & \UseMacro{ds-CG-train-T_num-data}
 & \UseMacro{ds-CG-val-T_num-data}
 & \UseMacro{ds-CG-test_standard-T_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (CGT-base) {\phantom{XX}};
 & \UseMacro{TH-ds-CP-T}
 & \UseMacro{ds-CG-test_common-CP-T_num-data}
\\
\midrule
 & \UseMacro{TH-ds-MP}
 & \UseMacro{ds-MN-train-MP_num-data}
 & \UseMacro{ds-MN-val-MP_num-data}
 & \UseMacro{ds-MN-test_standard-MP_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (MNMP-base) {\phantom{XX}};
 & \UseMacro{TH-ds-MP-CP}
 & \UseMacro{ds-MN-test_common-MP-CP_num-data}
\\
 & \UseMacro{TH-ds-CP}
 & \UseMacro{ds-MN-train-CP_num-data}
 & \UseMacro{ds-MN-val-CP_num-data}
 & \UseMacro{ds-MN-test_standard-CP_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (MNCP-base) {\phantom{XX}};
 & \UseMacro{TH-ds-MP-T}
 & \UseMacro{ds-MN-test_common-MP-T_num-data}
\\
\multirow{-3.5}{*}{\rotatebox[origin=c]{90}{\UseMacro{TaskM_MN}}}
 & \UseMacro{TH-ds-T}
 & \UseMacro{ds-MN-train-T_num-data}
 & \UseMacro{ds-MN-val-T_num-data}
 & \UseMacro{ds-MN-test_standard-T_num-data}
 & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0, yshift=1ex] (MNT-base) {\phantom{XX}};
 & \UseMacro{TH-ds-CP-T}
 & \UseMacro{ds-MN-test_common-CP-T_num-data}
\\
\bottomrule
\end{tabular}
\begin{tikzpicture}[remember picture, overlay, thick]
\draw[->] (CGMP-base.west) .. controls ($(CGMP-base.east) - (1em,0)$) .. (CGMP-base.east);
\draw (CGCP-base.west) .. controls ($(CGMP-base.east) - (1em,0)$) .. (CGMP-base.east);
\draw[->] (CGMP-base.west) .. controls ($(CGCP-base.east) - (1em,0)$) .. (CGCP-base.east);
\draw (CGT-base.west) .. controls ($(CGCP-base.east) - (1em,0)$) .. (CGCP-base.east);
\draw[->] (CGCP-base.west) .. controls ($(CGT-base.east) - (1em,0)$) .. (CGT-base.east);
\draw (CGT-base.west) .. controls ($(CGT-base.east) - (1em,0)$) .. (CGT-base.east);
\draw[->] (MNMP-base.west) .. controls ($(MNMP-base.east) - (1em,0)$) .. (MNMP-base.east);
\draw (MNCP-base.west) .. controls ($(MNMP-base.east) - (1em,0)$) .. (MNMP-base.east);
\draw[->] (MNMP-base.west) .. controls ($(MNCP-base.east) - (1em,0)$) .. (MNCP-base.east);
\draw (MNT-base.west) .. controls ($(MNCP-base.east) - (1em,0)$) .. (MNCP-base.east);
\draw[->] (MNCP-base.west) .. controls ($(MNT-base.east) - (1em,0)$) .. (MNT-base.east);
\draw (MNT-base.west) .. controls ($(MNT-base.east) - (1em,0)$) .. (MNT-base.east);
\end{tikzpicture}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-dataset-metrics-small}}
\caption{\UseMacro{TC-dataset-metrics-small}}
\end{table}


==> tables/table-dataset-metrics.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}
\begin{small}
\begin{center}
\caption{\TCDatasetMetrics}
\begin{tabular}{ l@{\hspace{2pt}}|@{\hspace{2pt}}c@{\hspace{2pt}} | r@{\hspace{8pt}} r@{\hspace{8pt}}r@{\hspace{8pt}}r @{\hspace{5pt}}c@{\hspace{5pt}} r@{\hspace{8pt}}r@{\hspace{8pt}}r @{\hspace{5pt}}c@{\hspace{5pt}} r@{\hspace{8pt}}r@{\hspace{8pt}}r @{\hspace{5pt}}c@{\hspace{5pt}} r@{\hspace{8pt}}r@{\hspace{8pt}}rr@{}}
\toprule
\multicolumn{2}{c|}{} & & \multicolumn{3}{c}{\UseMacro{TH-ds-MP-NT}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-CP-NT}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-MP-T}} & & \multicolumn{3}{c}{\UseMacro{TH-ds-CP-T}} & \\\cline{4-6}\cline{8-10}\cline{12-14}\cline{16-18}
\multicolumn{2}{c|}{\multirow{-2}{*}{\THDSStat}} & \multirow{-2}{*}{\UseMacro{TH-ds-all}} & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & & \UseMacro{TH-ds-train} & \UseMacro{TH-ds-val} & \UseMacro{TH-ds-test_standard} & \multirow{-2}{*}{\UseMacro{TH-ds-test_common}} \\
\midrule
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-project}}
 & \UseMacro{ds-num_prj_all}
 & \UseMacro{ds-num_prj_all}
 & \UseMacro{ds-num_prj_all}
 & \UseMacro{ds-num_prj_all}
 & 
 & \UseMacro{ds-num_prj_train}
 & \UseMacro{ds-num_prj_val}
 & \UseMacro{ds-num_prj_test}
 & 
 & \UseMacro{ds-num_prj_all}
 & \UseMacro{ds-num_prj_all}
 & \UseMacro{ds-num_prj_all}
 & 
 & \UseMacro{ds-num_prj_train}
 & \UseMacro{ds-num_prj_val}
 & \UseMacro{ds-num_prj_test}
 & \UseMacro{ds-num_prj_test}
\\
\multicolumn{2}{c|}{\UseMacro{TH-ds-num-data}}
 & \UseMacro{ds-all_num-data}
 & \UseMacro{ds-MP-NT-train_num-data}
 & \UseMacro{ds-MP-NT-val_num-data}
 & \UseMacro{ds-MP-NT-test_standard_num-data}
 & 
 & \UseMacro{ds-CP-NT-train_num-data}
 & \UseMacro{ds-CP-NT-val_num-data}
 & \UseMacro{ds-CP-NT-test_standard_num-data}
 & 
 & \UseMacro{ds-MP-T-train_num-data}
 & \UseMacro{ds-MP-T-val_num-data}
 & \UseMacro{ds-MP-T-test_standard_num-data}
 & 
 & \UseMacro{ds-CP-T-train_num-data}
 & \UseMacro{ds-CP-T-val_num-data}
 & \UseMacro{ds-CP-T-test_standard_num-data}
 & \UseMacro{ds-MP-NT-test_common_num-data}
\\
\midrule
& \UseMacro{TH-ds-len-method-avg}
 & \UseMacro{ds-all_len-meth-AVG}
 & \UseMacro{ds-MP-NT-train_len-meth-AVG}
 & \UseMacro{ds-MP-NT-val_len-meth-AVG}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-AVG}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-AVG}
 & \UseMacro{ds-CP-NT-val_len-meth-AVG}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-AVG}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-AVG}
 & \UseMacro{ds-MP-T-val_len-meth-AVG}
 & \UseMacro{ds-MP-T-test_standard_len-meth-AVG}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-AVG}
 & \UseMacro{ds-CP-T-val_len-meth-AVG}
 & \UseMacro{ds-CP-T-test_standard_len-meth-AVG}
 & \UseMacro{ds-MP-NT-test_common_len-meth-AVG}
\\
& \UseMacro{TH-ds-len-method-mode}
 & \UseMacro{ds-all_len-meth-MODE}
 & \UseMacro{ds-MP-NT-train_len-meth-MODE}
 & \UseMacro{ds-MP-NT-val_len-meth-MODE}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-MODE}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-MODE}
 & \UseMacro{ds-CP-NT-val_len-meth-MODE}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-MODE}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-MODE}
 & \UseMacro{ds-MP-T-val_len-meth-MODE}
 & \UseMacro{ds-MP-T-test_standard_len-meth-MODE}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-MODE}
 & \UseMacro{ds-CP-T-val_len-meth-MODE}
 & \UseMacro{ds-CP-T-test_standard_len-meth-MODE}
 & \UseMacro{ds-MP-NT-test_common_len-meth-MODE}
\\
& \UseMacro{TH-ds-len-method-median}
 & \UseMacro{ds-all_len-meth-MEDIAN}
 & \UseMacro{ds-MP-NT-train_len-meth-MEDIAN}
 & \UseMacro{ds-MP-NT-val_len-meth-MEDIAN}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-MEDIAN}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-MEDIAN}
 & \UseMacro{ds-CP-NT-val_len-meth-MEDIAN}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-MEDIAN}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-MEDIAN}
 & \UseMacro{ds-MP-T-val_len-meth-MEDIAN}
 & \UseMacro{ds-MP-T-test_standard_len-meth-MEDIAN}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-MEDIAN}
 & \UseMacro{ds-CP-T-val_len-meth-MEDIAN}
 & \UseMacro{ds-CP-T-test_standard_len-meth-MEDIAN}
 & \UseMacro{ds-MP-NT-test_common_len-meth-MEDIAN}
\\
& \UseMacro{TH-ds-len-method-le100}
 & \UseMacro{ds-all_len-meth-le-100}
 & \UseMacro{ds-MP-NT-train_len-meth-le-100}
 & \UseMacro{ds-MP-NT-val_len-meth-le-100}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-le-100}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-le-100}
 & \UseMacro{ds-CP-NT-val_len-meth-le-100}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-le-100}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-le-100}
 & \UseMacro{ds-MP-T-val_len-meth-le-100}
 & \UseMacro{ds-MP-T-test_standard_len-meth-le-100}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-le-100}
 & \UseMacro{ds-CP-T-val_len-meth-le-100}
 & \UseMacro{ds-CP-T-test_standard_len-meth-le-100}
 & \UseMacro{ds-MP-NT-test_common_len-meth-le-100}
\\
& \UseMacro{TH-ds-len-method-le150}
 & \UseMacro{ds-all_len-meth-le-150}
 & \UseMacro{ds-MP-NT-train_len-meth-le-150}
 & \UseMacro{ds-MP-NT-val_len-meth-le-150}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-le-150}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-le-150}
 & \UseMacro{ds-CP-NT-val_len-meth-le-150}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-le-150}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-le-150}
 & \UseMacro{ds-MP-T-val_len-meth-le-150}
 & \UseMacro{ds-MP-T-test_standard_len-meth-le-150}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-le-150}
 & \UseMacro{ds-CP-T-val_len-meth-le-150}
 & \UseMacro{ds-CP-T-test_standard_len-meth-le-150}
 & \UseMacro{ds-MP-NT-test_common_len-meth-le-150}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-method}} & \UseMacro{TH-ds-len-method-le200}
 & \UseMacro{ds-all_len-meth-le-200}
 & \UseMacro{ds-MP-NT-train_len-meth-le-200}
 & \UseMacro{ds-MP-NT-val_len-meth-le-200}
 & \UseMacro{ds-MP-NT-test_standard_len-meth-le-200}
 & 
 & \UseMacro{ds-CP-NT-train_len-meth-le-200}
 & \UseMacro{ds-CP-NT-val_len-meth-le-200}
 & \UseMacro{ds-CP-NT-test_standard_len-meth-le-200}
 & 
 & \UseMacro{ds-MP-T-train_len-meth-le-200}
 & \UseMacro{ds-MP-T-val_len-meth-le-200}
 & \UseMacro{ds-MP-T-test_standard_len-meth-le-200}
 & 
 & \UseMacro{ds-CP-T-train_len-meth-le-200}
 & \UseMacro{ds-CP-T-val_len-meth-le-200}
 & \UseMacro{ds-CP-T-test_standard_len-meth-le-200}
 & \UseMacro{ds-MP-NT-test_common_len-meth-le-200}
\\
\midrule
& \UseMacro{TH-ds-len-comment-avg}
 & \UseMacro{ds-all_len-com-AVG}
 & \UseMacro{ds-MP-NT-train_len-com-AVG}
 & \UseMacro{ds-MP-NT-val_len-com-AVG}
 & \UseMacro{ds-MP-NT-test_standard_len-com-AVG}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-AVG}
 & \UseMacro{ds-CP-NT-val_len-com-AVG}
 & \UseMacro{ds-CP-NT-test_standard_len-com-AVG}
 & 
 & \UseMacro{ds-MP-T-train_len-com-AVG}
 & \UseMacro{ds-MP-T-val_len-com-AVG}
 & \UseMacro{ds-MP-T-test_standard_len-com-AVG}
 & 
 & \UseMacro{ds-CP-T-train_len-com-AVG}
 & \UseMacro{ds-CP-T-val_len-com-AVG}
 & \UseMacro{ds-CP-T-test_standard_len-com-AVG}
 & \UseMacro{ds-MP-NT-test_common_len-com-AVG}
\\
& \UseMacro{TH-ds-len-comment-mode}
 & \UseMacro{ds-all_len-com-MODE}
 & \UseMacro{ds-MP-NT-train_len-com-MODE}
 & \UseMacro{ds-MP-NT-val_len-com-MODE}
 & \UseMacro{ds-MP-NT-test_standard_len-com-MODE}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-MODE}
 & \UseMacro{ds-CP-NT-val_len-com-MODE}
 & \UseMacro{ds-CP-NT-test_standard_len-com-MODE}
 & 
 & \UseMacro{ds-MP-T-train_len-com-MODE}
 & \UseMacro{ds-MP-T-val_len-com-MODE}
 & \UseMacro{ds-MP-T-test_standard_len-com-MODE}
 & 
 & \UseMacro{ds-CP-T-train_len-com-MODE}
 & \UseMacro{ds-CP-T-val_len-com-MODE}
 & \UseMacro{ds-CP-T-test_standard_len-com-MODE}
 & \UseMacro{ds-MP-NT-test_common_len-com-MODE}
\\
& \UseMacro{TH-ds-len-comment-median}
 & \UseMacro{ds-all_len-com-MEDIAN}
 & \UseMacro{ds-MP-NT-train_len-com-MEDIAN}
 & \UseMacro{ds-MP-NT-val_len-com-MEDIAN}
 & \UseMacro{ds-MP-NT-test_standard_len-com-MEDIAN}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-MEDIAN}
 & \UseMacro{ds-CP-NT-val_len-com-MEDIAN}
 & \UseMacro{ds-CP-NT-test_standard_len-com-MEDIAN}
 & 
 & \UseMacro{ds-MP-T-train_len-com-MEDIAN}
 & \UseMacro{ds-MP-T-val_len-com-MEDIAN}
 & \UseMacro{ds-MP-T-test_standard_len-com-MEDIAN}
 & 
 & \UseMacro{ds-CP-T-train_len-com-MEDIAN}
 & \UseMacro{ds-CP-T-val_len-com-MEDIAN}
 & \UseMacro{ds-CP-T-test_standard_len-com-MEDIAN}
 & \UseMacro{ds-MP-NT-test_common_len-com-MEDIAN}
\\
& \UseMacro{TH-ds-len-comment-le20}
 & \UseMacro{ds-all_len-com-le-20}
 & \UseMacro{ds-MP-NT-train_len-com-le-20}
 & \UseMacro{ds-MP-NT-val_len-com-le-20}
 & \UseMacro{ds-MP-NT-test_standard_len-com-le-20}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-le-20}
 & \UseMacro{ds-CP-NT-val_len-com-le-20}
 & \UseMacro{ds-CP-NT-test_standard_len-com-le-20}
 & 
 & \UseMacro{ds-MP-T-train_len-com-le-20}
 & \UseMacro{ds-MP-T-val_len-com-le-20}
 & \UseMacro{ds-MP-T-test_standard_len-com-le-20}
 & 
 & \UseMacro{ds-CP-T-train_len-com-le-20}
 & \UseMacro{ds-CP-T-val_len-com-le-20}
 & \UseMacro{ds-CP-T-test_standard_len-com-le-20}
 & \UseMacro{ds-MP-NT-test_common_len-com-le-20}
\\
& \UseMacro{TH-ds-len-comment-le30}
 & \UseMacro{ds-all_len-com-le-30}
 & \UseMacro{ds-MP-NT-train_len-com-le-30}
 & \UseMacro{ds-MP-NT-val_len-com-le-30}
 & \UseMacro{ds-MP-NT-test_standard_len-com-le-30}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-le-30}
 & \UseMacro{ds-CP-NT-val_len-com-le-30}
 & \UseMacro{ds-CP-NT-test_standard_len-com-le-30}
 & 
 & \UseMacro{ds-MP-T-train_len-com-le-30}
 & \UseMacro{ds-MP-T-val_len-com-le-30}
 & \UseMacro{ds-MP-T-test_standard_len-com-le-30}
 & 
 & \UseMacro{ds-CP-T-train_len-com-le-30}
 & \UseMacro{ds-CP-T-val_len-com-le-30}
 & \UseMacro{ds-CP-T-test_standard_len-com-le-30}
 & \UseMacro{ds-MP-NT-test_common_len-com-le-30}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-comment}} & \UseMacro{TH-ds-len-comment-le50}
 & \UseMacro{ds-all_len-com-le-50}
 & \UseMacro{ds-MP-NT-train_len-com-le-50}
 & \UseMacro{ds-MP-NT-val_len-com-le-50}
 & \UseMacro{ds-MP-NT-test_standard_len-com-le-50}
 & 
 & \UseMacro{ds-CP-NT-train_len-com-le-50}
 & \UseMacro{ds-CP-NT-val_len-com-le-50}
 & \UseMacro{ds-CP-NT-test_standard_len-com-le-50}
 & 
 & \UseMacro{ds-MP-T-train_len-com-le-50}
 & \UseMacro{ds-MP-T-val_len-com-le-50}
 & \UseMacro{ds-MP-T-test_standard_len-com-le-50}
 & 
 & \UseMacro{ds-CP-T-train_len-com-le-50}
 & \UseMacro{ds-CP-T-val_len-com-le-50}
 & \UseMacro{ds-CP-T-test_standard_len-com-le-50}
 & \UseMacro{ds-MP-NT-test_common_len-com-le-50}
\\
\midrule
& \UseMacro{TH-ds-len-name-avg}
 & \UseMacro{ds-all_len-name-AVG}
 & \UseMacro{ds-MP-NT-train_len-name-AVG}
 & \UseMacro{ds-MP-NT-val_len-name-AVG}
 & \UseMacro{ds-MP-NT-test_standard_len-name-AVG}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-AVG}
 & \UseMacro{ds-CP-NT-val_len-name-AVG}
 & \UseMacro{ds-CP-NT-test_standard_len-name-AVG}
 & 
 & \UseMacro{ds-MP-T-train_len-name-AVG}
 & \UseMacro{ds-MP-T-val_len-name-AVG}
 & \UseMacro{ds-MP-T-test_standard_len-name-AVG}
 & 
 & \UseMacro{ds-CP-T-train_len-name-AVG}
 & \UseMacro{ds-CP-T-val_len-name-AVG}
 & \UseMacro{ds-CP-T-test_standard_len-name-AVG}
 & \UseMacro{ds-MP-NT-test_common_len-name-AVG}
\\
& \UseMacro{TH-ds-len-name-mode}
 & \UseMacro{ds-all_len-name-MODE}
 & \UseMacro{ds-MP-NT-train_len-name-MODE}
 & \UseMacro{ds-MP-NT-val_len-name-MODE}
 & \UseMacro{ds-MP-NT-test_standard_len-name-MODE}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-MODE}
 & \UseMacro{ds-CP-NT-val_len-name-MODE}
 & \UseMacro{ds-CP-NT-test_standard_len-name-MODE}
 & 
 & \UseMacro{ds-MP-T-train_len-name-MODE}
 & \UseMacro{ds-MP-T-val_len-name-MODE}
 & \UseMacro{ds-MP-T-test_standard_len-name-MODE}
 & 
 & \UseMacro{ds-CP-T-train_len-name-MODE}
 & \UseMacro{ds-CP-T-val_len-name-MODE}
 & \UseMacro{ds-CP-T-test_standard_len-name-MODE}
 & \UseMacro{ds-MP-NT-test_common_len-name-MODE}
\\
& \UseMacro{TH-ds-len-name-median}
 & \UseMacro{ds-all_len-name-MEDIAN}
 & \UseMacro{ds-MP-NT-train_len-name-MEDIAN}
 & \UseMacro{ds-MP-NT-val_len-name-MEDIAN}
 & \UseMacro{ds-MP-NT-test_standard_len-name-MEDIAN}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-MEDIAN}
 & \UseMacro{ds-CP-NT-val_len-name-MEDIAN}
 & \UseMacro{ds-CP-NT-test_standard_len-name-MEDIAN}
 & 
 & \UseMacro{ds-MP-T-train_len-name-MEDIAN}
 & \UseMacro{ds-MP-T-val_len-name-MEDIAN}
 & \UseMacro{ds-MP-T-test_standard_len-name-MEDIAN}
 & 
 & \UseMacro{ds-CP-T-train_len-name-MEDIAN}
 & \UseMacro{ds-CP-T-val_len-name-MEDIAN}
 & \UseMacro{ds-CP-T-test_standard_len-name-MEDIAN}
 & \UseMacro{ds-MP-NT-test_common_len-name-MEDIAN}
\\
& \UseMacro{TH-ds-len-name-le2}
 & \UseMacro{ds-all_len-name-le-3}
 & \UseMacro{ds-MP-NT-train_len-name-le-3}
 & \UseMacro{ds-MP-NT-val_len-name-le-3}
 & \UseMacro{ds-MP-NT-test_standard_len-name-le-3}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-le-3}
 & \UseMacro{ds-CP-NT-val_len-name-le-3}
 & \UseMacro{ds-CP-NT-test_standard_len-name-le-3}
 & 
 & \UseMacro{ds-MP-T-train_len-name-le-3}
 & \UseMacro{ds-MP-T-val_len-name-le-3}
 & \UseMacro{ds-MP-T-test_standard_len-name-le-3}
 & 
 & \UseMacro{ds-CP-T-train_len-name-le-3}
 & \UseMacro{ds-CP-T-val_len-name-le-3}
 & \UseMacro{ds-CP-T-test_standard_len-name-le-3}
 & \UseMacro{ds-MP-NT-test_common_len-name-le-3}
\\
& \UseMacro{TH-ds-len-name-le3}
 & \UseMacro{ds-all_len-name-le-5}
 & \UseMacro{ds-MP-NT-train_len-name-le-5}
 & \UseMacro{ds-MP-NT-val_len-name-le-5}
 & \UseMacro{ds-MP-NT-test_standard_len-name-le-5}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-le-5}
 & \UseMacro{ds-CP-NT-val_len-name-le-5}
 & \UseMacro{ds-CP-NT-test_standard_len-name-le-5}
 & 
 & \UseMacro{ds-MP-T-train_len-name-le-5}
 & \UseMacro{ds-MP-T-val_len-name-le-5}
 & \UseMacro{ds-MP-T-test_standard_len-name-le-5}
 & 
 & \UseMacro{ds-CP-T-train_len-name-le-5}
 & \UseMacro{ds-CP-T-val_len-name-le-5}
 & \UseMacro{ds-CP-T-test_standard_len-name-le-5}
 & \UseMacro{ds-MP-NT-test_common_len-name-le-5}
\\
\multirow{-6}{*}{\UseMacro{TH-ds-len-name}} & \UseMacro{TH-ds-len-name-le6}
 & \UseMacro{ds-all_len-name-le-6}
 & \UseMacro{ds-MP-NT-train_len-name-le-6}
 & \UseMacro{ds-MP-NT-val_len-name-le-6}
 & \UseMacro{ds-MP-NT-test_standard_len-name-le-6}
 & 
 & \UseMacro{ds-CP-NT-train_len-name-le-6}
 & \UseMacro{ds-CP-NT-val_len-name-le-6}
 & \UseMacro{ds-CP-NT-test_standard_len-name-le-6}
 & 
 & \UseMacro{ds-MP-T-train_len-name-le-6}
 & \UseMacro{ds-MP-T-val_len-name-le-6}
 & \UseMacro{ds-MP-T-test_standard_len-name-le-6}
 & 
 & \UseMacro{ds-CP-T-train_len-name-le-6}
 & \UseMacro{ds-CP-T-val_len-name-le-6}
 & \UseMacro{ds-CP-T-test_standard_len-name-le-6}
 & \UseMacro{ds-MP-NT-test_common_len-name-le-6}
\\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vspace{\TVDatasetMetrics}
\end{table*}


==> tables/table-eval-settings.tex <==
% Manually written

{\def\arraystretch{2}
\begin{table*}[t]
  \begin{scriptsize}
  \begin{center}
  \begin{tabular}{ | @{\hspace{2pt}}c@{\hspace{2pt}} | @{\hspace{2pt}}c@{\hspace{2pt}} | @{\hspace{3pt}}c@{\hspace{3pt}} |@{}c@{}| @{\hspace{2pt}}c@{\hspace{2pt}} | @{\hspace{2pt}}c@{\hspace{2pt}} | @{\hspace{3pt}}c@{\hspace{3pt}} | }
    \cline{1-3} \cline{5-7}
    \textbf{\makecell[c]{Metho-\\dology}} & \textbf{Set} & \textbf{Formula}
    & &
    \textbf{Pair} & \textbf{Set} & \textbf{Formula} \\
    \cline{1-3} \cline{5-7}
    & & & & & & \\[-4ex]
    \cline{1-3} \cline{5-7}

    % MP - MPxCP
    \rule{0pt}{3ex}
    & \textbf{\ATrain}
    & $\bigcup_{\aproject \in \aprojects} (\aexamples_{train}^{\atimepp, \aproject} \sunion \aexamples_{train}^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples_{train}^{\atime\setminus\atimep, \aproject})$
    &
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    & \textbf{\AVal}
    & $\bigcup_{\aproject \in \aprojects} (\aexamples_{val}^{\atimepp, \aproject} \sunion \aexamples_{val}^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples_{val}^{\atime\setminus\atimep, \aproject})$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (mpxcp-base) {\phantom{XX}};
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    \multirow{-3}{*}{\textbf{\Amp}}
    & \textbf{\ATestS}
    & $\bigcup_{\aproject \in \aprojects} (\aexamples_{test}^{\atimepp, \aproject} \sunion \aexamples_{test}^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples_{test}^{\atime\setminus\atimep, \aproject})$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (mp-base) {\phantom{XX}};
    & \multirow{-3}{*}{\textbf{\mpxcp}}
    & \multirow{-3}{*}{\textbf{\ATestC}}
    & \multirow{-3}{*}{$\bigcup_{\aproject \in \aprojects_{test}} (\aexamples_{test}^{\atimepp, \aproject} \sunion \aexamples_{test}^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples_{test}^{\atime\setminus\atimep, \aproject})$} \\
    \cline{1-3} \cline{5-7}
    & & & & & & \\[-4ex]
    \cline{1-3} \cline{5-7}


    % CP - MPxT
    \rule{0pt}{3ex}
    & \textbf{\ATrain}
    & $\bigcup_{\aproject \in \aprojects_{train}} (\aexamples^{\atimepp, \aproject} \sunion \aexamples^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples^{\atime\setminus\atimep, \aproject})$
    &
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    & \textbf{\AVal}
    & $\bigcup_{\aproject \in \aprojects_{val}} (\aexamples^{\atimepp, \aproject} \sunion \aexamples^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples^{\atime\setminus\atimep, \aproject})$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (mpxt-base) {\phantom{XX}};
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    \multirow{-3}{*}{\textbf{\Acp}}
    & \textbf{\ATestS}
    & $\bigcup_{\aproject \in \aprojects_{test}} (\aexamples^{\atimepp, \aproject} \sunion \aexamples^{\atimep\setminus\atimepp, \aproject} \sunion \aexamples^{\atime\setminus\atimep, \aproject})$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (cp-base) {\phantom{XX}};
    & \multirow{-3}{*}{\textbf{\mpxt}}
    & \multirow{-3}{*}{\textbf{\ATestC}}
    & \multirow{-3}{*}{$\bigcup_{\aproject \in \aprojects} \aexamples_{test}^{\atime\setminus\atimep, \aproject}$} \\
    \cline{1-3} \cline{5-7}
    & & & & & & \\[-4ex]
    \cline{1-3} \cline{5-7}


    % T - CPxT
    \rule{0pt}{3ex}
    & \textbf{\ATrain}
    & $\bigcup_{\aproject \in \aprojects} \aexamples^{\atimepp, \aproject}$
    &
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    & \textbf{\AVal}
    & $\bigcup_{\aproject \in \aprojects} \aexamples^{\atimep\setminus\atimepp, \aproject}$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (cpxt-base) {\phantom{XX}};
    &
    &
    & \\
    \cline{2-3}

    \rule{0pt}{3ex}
    \multirow{-3}{*}{\textbf{\At}}
    & \textbf{\ATestS}
    & $\bigcup_{\aproject \in \aprojects} \aexamples^{\atime\setminus\atimep, \aproject}$
    & \tikz[remember picture, baseline] \node[inner sep=2pt, outer sep=0] (t-base) {\phantom{XX}};
    & \multirow{-3}{*}{\textbf{\cpxt}}
    & \multirow{-3}{*}{\textbf{\ATestC}}
    & \multirow{-3}{*}{$\bigcup_{\aproject \in \aprojects_{test}} \aexamples^{\atime\setminus\atimep, \aproject}$} \\
    \cline{1-3} \cline{5-7}

  \end{tabular}

  \begin{tikzpicture}[remember picture, overlay, thick]
    \draw[->] (mp-base.west) .. controls ($(mpxcp-base.east) - (1em,0)$) .. (mpxcp-base.east);
    \draw[] (cp-base.west) .. controls ($(mpxcp-base.east) - (1em,0)$) .. (mpxcp-base.east);
    \draw[->] (mp-base.west) .. controls ($(mpxt-base.east) - (1em,0)$) .. (mpxt-base.east);
    \draw[] (t-base.west) .. controls ($(mpxt-base.east) - (1em,0)$) .. (mpxt-base.east);
    \draw[->] (cp-base.west) .. controls ($(cpxt-base.east) - (1em,0)$) .. (cpxt-base.east);
    \draw[] (t-base.west) .. controls ($(cpxt-base.east) - (1em,0)$) .. (cpxt-base.east);
  \end{tikzpicture}

  \end{center}
  \end{scriptsize}
  \caption{\TCEvalSettings}
  \vspace{\TVEvalSettings}
\end{table*}
}

==> tables/table-models.tex <==
\begin{table*}
\begin{scriptsize}
\begin{center}
\caption{\TCModels}
\begin{tabular}{l | l | l | l}

\toprule

Model & \makecell{Target\\Language} & Inputs & Code \\

\midrule

Iyer et al.~\cite{IyerETAL16Summarizing} CODE-NN &
\Csharp SQL &
code snippets &
\href{https://github.com/sriniiyer/codenn}{[Torch]} \\
\midrule

Liang and Zhu et al.~\cite{LiangAndZhu18Automatic} Tree-LSTM-GRU &
Java &
AST(exclude method names and params) &
\href{https://github.com/liang2024086/code_comment_generation}{[Tensorflow]} \\
\midrule

Wan et al.~\cite{WanETAL18SummarizationRL} Code-RL &
Python &
AST+code snippets &
\href{https://github.com/wanyao1992/code_Summarization_public}{[Pytorch]} \\
\midrule

Hu et al.~\cite{HuETAL18Deep} DeepCom &
Java &
SBT+code snippets &
\href{https://github.com/xing-hu/EMSE-DeepCom}{[Tensorflow]} \\
\midrule

Hu et al.~\cite{HuETAL18Summarizing} TL-CodeSum &
Java &
api sequence+code snippets &
\href{https://github.com/xing-hu/TL-CodeSum}{[Tensorflow]} \\
\midrule

LeClair et al.~\cite{LeClairETAL19Neural} ast-attendgru &
Java &
AST+code snippets &
\href{https://s3.us-east-2.amazonaws.com/icse2018/index.html}{[Keras]} \\
\midrule

Alon et al.~\cite{AlonETAL19Code2seq} Code2seq &
Java &
AST paths &
\href{https://github.com/m3yrin/Code2seq}{[Pytorch]} \\
\midrule

Fernandes et al.~\cite{FernandesETAL19Summarization} BiLSTM+GNN &
Java &
graph representation of code &
\href{https://github.com/CoderPat/structured-neural-summarization}{[Tensorflow]}\\
\midrule

LeClair et al.~\cite{LeClairETAL20Summarization} code+gnn+BiLSTM &
Java &
AST+code snippets &
\href{https://github.com/acleclair/ICPC2020_GNN}{[Tensorflow+Keras]} \\
\midrule

\bottomrule

\end{tabular}
\end{center}
\end{scriptsize}
\vspace{\TVModels}
\end{table*}


==> tables/table-prelim.tex <==
% Manually written

\begin{table}[t]
\begin{footnotesize}
  \centering
  \begin{tabular}{@{\hspace{2pt}} l @{\hspace{5pt}} p{5.7cm} @{\hspace{2pt}}}
    \toprule
    \textbf{Symbol} &
    \textbf{Definition} \\
    \midrule

    \atime, \atimep, \atimepp &

    Timestamps, i.e., specific points in time.  \atimepp is earlier
    than \atimep, and \atimep is earlier than \atime ($\atimepp <
    \atimep < \atime$).\\

    \midrule

    \aprojects &

    A set of projects, from which \examples are derived.\\

    \aproject &

    A project.\\

    \midrule

    \aexamples &

    A set of \examples.\\  % (e.g., \codecom pairs for the \comgen task).\\

    $\aexamples^{\atime, \aproject}$ &

    The set of \examples extracted from project \aproject at timestamp
    \atime.\\

    $\aexamples^{\atime\setminus\atimep, \aproject}$ &

    $= \aexamples^{\atime, \aproject} \setminus \aexamples^{\atimep,
      \aproject}$ (where $\setminus$ is the set difference operator),
    i.e., the \examples extracted from project \aproject at timestamp
    \atime that were not available at timestamp \atimep.\\

    \midrule

    $\ashuffle(l)$ &

    Given a set (of \examples or projects) $s$, returns a set with
    the same items after random shuffling.\\

    \midrule

    \makecell[lt]{$\asplit(\aexamples,$\\$\apcttrain, \apctval, \apcttest)$} &

    Given a set of \examples $\aexamples$, splits the set into three
    sets $\aexamples_x, \aexamples_y, \aexamples_z$ such that $\left|
    \aexamples_x \right| : \left| \aexamples_y \right| : \left|
    \aexamples_z \right| \approx \apcttrain:\apctval:\apcttest$;
    requires that $\apcttrain + \apctval + \apcttest = 1$.\\

    \midrule

    \makecell[lt]{$\asplitprj(\aprojects,$\\$\atime, \apcttrain, \apctval, \apcttest)$} &

    Given a set of projects $\aprojects$, splits the set into three
    sets $\aprojects_x, \aprojects_y, \aprojects_z$ such that

    $ \left| \bigcup_{p\in\aprojects_x}{\aexamples^{\atime, p}} \right|
    : \left| \bigcup_{p\in\aprojects_y}{\aexamples^{\atime, p}} \right|
    : \left| \bigcup_{p\in\aprojects_z}{\aexamples^{\atime, p}} \right|
    \approx \apcttrain:\apctval:\apcttest$; requires that $\apcttrain +
    \apctval + \apcttest = 1$.\\

    \bottomrule
  \end{tabular}
  \caption{\TCPrelim}
  \vspace{\TVPrelim}
\end{footnotesize}
\end{table}


==> tables/table-prior-work-code-sum.tex <==
% Manually written

\begin{table*}[t]
\begin{footnotesize}
  \centering
  \begin{tabular}{@{}l | l@{\hspace{5pt}}l@{\hspace{6pt}}l@{\hspace{5pt}}>{\scriptsize}l c@{\hspace{5pt}}c@{\hspace{3pt}}c}
    \toprule
    & & & & & \multicolumn{3}{c}{\textbf{\Methodology}} \\\cline{6-8}
    \multirow{-2}{*}{\textbf{Task}} &
    \multirow{-2}{*}{\textbf{Reference}} &
    \multirow{-2}{*}{\textbf{Published at}} &
    \multirow{-2}{*}{\textbf{Language}} &
    \multirow{-2}{*}{\footnotesize\textbf{Automatic Metrics}} &
    \textbf{\Amp} & \textbf{\Acp} & \textbf{\At} \\
    \midrule

    & \citet{IyerETAL16Summarizing} & ACL'16 & \Csharp, SQL & \BLEU, \METEOR & \mycheckmark & \mycross & \mycross \\
    & \citet{WanETAL18SummarizationRL} & ASE'18 & Python & \BLEU, \METEOR, \ROUGEf, CIDER & \mycheckmark & \mycross & \mycross \\ % 2018 Sep
    & \citet{XuETAL18Graph2Seq} & EMNLP'18 & SQL & \BLEU & \mycheckmark & \mycross & \mycross \\ % 2018 Oct
    & \citet{FernandesETAL19Summarization} & ICLR'19 & \Csharp & \BLEU, \ROUGEf, ROUGE-2, \Fone & \mycheckmark & \mycross & \mycross \\ % 2019
    & \citet{LeClairETAL19Neural} & ICSE'19 & Java & \BLEU & \mycross & \mycheckmark & \mycross \\ % 2019 May
    \rowcolor{blue!10} \cellcolor{white} & \citet{HuETAL18Deep,HuETAL20DeepComHybrid} & ICPC'18, ESE'20 & Java & \BLEU, \METEOR, \Precision, \Recall, \Fone & \mycheckmark & \mycross & \mycross \\ % 2019 June
    & \citet{LeClairETAL20Summarization} & ICPC'20 & Java & \BLEU, \ROUGEf & \mycross & \mycheckmark & \mycross \\ % 2020 July
    & \citet{CaiETAL20TAG} & ACL'20 & SQL, Python & \BLEU, \ROUGEf, ROUGE-2 & \mycheckmark & \mycross & \mycross \\ % 2020 July
    \rowcolor{blue!10} \cellcolor{white} & \citet{AhmadETAL20Transformer} & ACL'20 & Java, Python & \BLEU, \METEOR, \ROUGEf & \mycheckmark & \mycross & \mycross \\ % 2020 July
    % \makecell[l]{\scriptsize Java, Python, Ruby,\\\scriptsize JavaScript, Go, PHP}
    & \citet{FengETAL20CodeBERT} & EMNLP'20 & Java, Python, etc. & \BLEU & \mycheckmark & \mycross & \mycross \\ % 2020 Nov
    \multirow{-11}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Comment\\Generation}}} & \citet{AhmadETAL21PLBART} & NAACL'21 & Java, Python, etc. & \BLEU & \mycheckmark & \mycross & \mycross \\ % 2021
    \midrule
    & \citet{AllamanisETAL16Convolutional} & ICML'16 & Java & \Precision, \Recall, \Fone, \XMatch & \mycheckmark & \mycross & \mycross \\
    & \citet{FernandesETAL19Summarization} & ICLR'19 & Java, \Csharp & \ROUGEf, ROUGE-2, \Fone & \mycheckmark & \mycross & \mycross \\ % 2019
    & \citet{XuETAL19Method} & PEPM'19 & Java & \Precision, \Recall, \Fone, \XMatch & \mycheckmark & \mycross & \mycross \\ % 2019 Jan
    \rowcolor{blue!10} \cellcolor{white} & \citet{AlonETAL19Code2vec} & POPL'19 & Java & \Precision, \Recall, \Fone & \mycheckmark & \mycross & \mycross \\ % 2019 Jan
    \rowcolor{blue!10} \cellcolor{white} & \citet{AlonETAL19Code2seq} & ICLR'19 & Java & \Precision, \Recall, \Fone & \mycross & \mycheckmark & \mycross \\ % 2019
    & \citet{YonaiETAL19Mercem} & APSEC'19 & Java & Top-10 Accuracy & \mycheckmark & \mycross & \mycross \\ % 2019 July
    \multirow{-7}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Method\\Naming}}} & \citet{NguyenETAL20MethodNames} & ICSE'20 & Java & \Precision, \Recall, \Fone & \mycheckmark & \mycheckmark & \mycross \\ % 2020 May
    \midrule
    Sum & \na & \na & \na & {\footnotesize\na} & \NumCodeSumMP & \NumCodeSumCP & \NumCodeSumT \\
    \bottomrule
  \end{tabular}
  \caption{\TCPriorWorkCodeSum}
  \vspace{\TVPriorWorkCodeSum}
\end{footnotesize}
\end{table*}



==> tables/table-prior-work-temporal.tex <==
% Manually written

\begin{table*}[t]
\begin{small}
  \centering
  \caption{\TCPriorWorkTemporal}
  \begin{tabular}{lllll}
    \toprule
    \textbf{Task} &
    \textbf{Authors} &
    \textbf{Reference} &
    \textbf{Published at} &
    \textbf{Notes}
    \\
    \midrule

    & D'Ambros et al. & \cite{DAmbrosETAL12DefectPrediction} & ESE'12 & \\ % a dataset
    & Tan et al. & \cite{TanETAL15Online} & ICSE'15 & \\
    & Wang et al. & \cite{WangETAL16DefectPrediction} & ICSE'16 & Cited~\cite{TanETAL15Online} \\
    \multirow{-3}{*}{Defect Prediction} & Kamei et al. & \cite{KameiETAL16JITDefectPrediction} & ESE'16 & Cited~\cite{TanETAL15Online} \\
    \midrule
    Program Repair & Lutellier et al. & \cite{LutellierETAL20CoCoNut} & ISSTA'20 & \\
    \midrule
    Bug Localization & Pradel et al. & \cite{PradelETAL20Scaffle} & ISSTA'20 & \\

    \bottomrule

  \end{tabular}
  \vspace{\TVPriorWorkTemporal}
\end{small}
\end{table*}


==> tables/table-results-CG.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_bleu}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_bleu}
 & $^{\beta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_bleu}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_bleu}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_bleu}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_bleu}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_bleu}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_bleu}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_bleu}
 & $^{\beta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_bleu}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_bleu}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_bleu}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_bleu}}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_bleu}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_bleu}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_bleu}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_bleu}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_bleu}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_meteor}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_meteor}
 & $^{\delta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_meteor}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_meteor}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_meteor}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_meteor}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_meteor}
 & $^{\gamma}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_meteor}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_meteor}
 & $^{\delta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_meteor}
 & $^{\epsilon}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_meteor}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_meteor}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_meteor}}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_meteor}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_meteor}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_meteor}}
 & $^{\epsilon}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_meteor}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_meteor}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_rouge_l_f}
 & $^{\zeta}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_rouge_l_f}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_rouge_l_f}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_rouge_l_f}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_rouge_l_f}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_rouge_l_f}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_rouge_l_f}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_rouge_l_f}
 & $^{\zeta}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_rouge_l_f}
 & \UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_rouge_l_f}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_rouge_l_f}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_rouge_l_f}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-CP_exact_match}
 & $^{\eta}$$^{\theta}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-MP-CP_exact_match}
 & $^{\kappa}$\UseMacro{result-CG_MP_DeepComHybridESE19_test_common-MP-T_exact_match}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-MP-T_exact_match}
 & $^{\lambda}$$^{\mu}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_common-CP-T_exact_match}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_common-CP-T_exact_match}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-CP_exact_match}
 & $^{\eta}$$^{\iota}$\UseMacro{result-CG_CP_RNNBaseline_test_common-MP-CP_exact_match}
 & \UseMacro{result-CG_MP_RNNBaseline_test_common-MP-T_exact_match}
 & $^{\kappa}$\UseMacro{result-CG_T_RNNBaseline_test_common-MP-T_exact_match}
 & $^{\lambda}$\UseMacro{result-CG_CP_RNNBaseline_test_common-CP-T_exact_match}
 & \UseMacro{result-CG_T_RNNBaseline_test_common-CP-T_exact_match}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-CP_exact_match}}
 & $^{\theta}$$^{\iota}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-MP-CP_exact_match}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_common-MP-T_exact_match}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-MP-T_exact_match}}
 & $^{\mu}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_common-CP-T_exact_match}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_common-CP-T_exact_match}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-CG}}
\caption{\UseMacro{TC-results-CG}}
\end{table}


==> tables/table-results-MN.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r | r@{\hspace{3pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-MP}}
 & \makecell[c]{\UseMacro{TH-T}}
 & \makecell[c]{\UseMacro{TH-CP}}
 & \makecell[c]{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-CP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP-T}}
 & \multicolumn{2}{c}{\UseMacro{TH-CP-T}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_p}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_p}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_p}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_p}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_p}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_p}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_p}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_p}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_p}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_p}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_p}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_p}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_r}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_r}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_r}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_r}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_r}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_r}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_r}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_r}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_r}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_r}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_r}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_r}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_set_match_f}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_set_match_f}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_set_match_f}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_set_match_f}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_set_match_f}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_set_match_f}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_set_match_f}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_set_match_f}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_set_match_f}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_set_match_f}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_set_match_f}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_set_match_f}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-CP_exact_match}}
 & $^{\alpha}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-MP-CP_exact_match}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_common-MP-T_exact_match}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-MP-T_exact_match}}
 & $^{\beta}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_common-CP-T_exact_match}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_common-CP-T_exact_match}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-CP_exact_match}
 & $^{\alpha}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-MP-CP_exact_match}}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_common-MP-T_exact_match}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-MP-T_exact_match}
 & $^{\beta}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_common-CP-T_exact_match}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_common-CP-T_exact_match}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-MN}}
\caption{\UseMacro{TC-results-MN}}
\end{table}


==> tables/table-results-aux-CG.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-bleu}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_bleu}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_bleu}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_bleu}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_bleu}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_bleu}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_bleu}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_bleu}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_bleu}
 & $^{\alpha}$\UseMacro{result-CG_CP_RNNBaseline_val_bleu}
 & $^{\beta}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_bleu}
 & \UseMacro{result-CG_T_RNNBaseline_val_bleu}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_bleu}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_val_bleu}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_bleu}}
 & $^{\alpha}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_val_bleu}}
 & $^{\beta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_bleu}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_val_bleu}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_bleu}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-meteor}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_meteor}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_meteor}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_meteor}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_meteor}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_meteor}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_meteor}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_meteor}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_meteor}
 & $^{\gamma}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_val_meteor}}
 & $^{\delta}$\textbf{\UseMacro{result-CG_CP_RNNBaseline_test_standard_meteor}}
 & \UseMacro{result-CG_T_RNNBaseline_val_meteor}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_meteor}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_val_meteor}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_meteor}}
 & $^{\gamma}$\UseMacro{result-CG_CP_TransformerACL20_val_meteor}
 & $^{\delta}$\UseMacro{result-CG_CP_TransformerACL20_test_standard_meteor}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_val_meteor}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_meteor}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-rouge_l_f}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_rouge_l_f}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_rouge_l_f}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_val_rouge_l_f}
 & \UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_rouge_l_f}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_rouge_l_f}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_rouge_l_f}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_rouge_l_f}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_rouge_l_f}
 & $^{\epsilon}$\UseMacro{result-CG_CP_RNNBaseline_val_rouge_l_f}
 & $^{\zeta}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_rouge_l_f}
 & \UseMacro{result-CG_T_RNNBaseline_val_rouge_l_f}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_rouge_l_f}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_val_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_rouge_l_f}}
 & $^{\epsilon}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_val_rouge_l_f}}
 & $^{\zeta}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_val_rouge_l_f}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_rouge_l_f}}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-DeepComHybridESE19}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_val_exact_match}
 & \UseMacro{result-CG_MP_DeepComHybridESE19_test_standard_exact_match}
 & $^{\eta}$\textbf{\UseMacro{result-CG_CP_DeepComHybridESE19_val_exact_match}}
 & $^{\theta}$$^{\iota}$\UseMacro{result-CG_CP_DeepComHybridESE19_test_standard_exact_match}
 & \UseMacro{result-CG_T_DeepComHybridESE19_val_exact_match}
 & \UseMacro{result-CG_T_DeepComHybridESE19_test_standard_exact_match}
\\
\UseMacro{TH-model-RNNBaseline}
 & \UseMacro{result-CG_MP_RNNBaseline_val_exact_match}
 & \UseMacro{result-CG_MP_RNNBaseline_test_standard_exact_match}
 & \UseMacro{result-CG_CP_RNNBaseline_val_exact_match}
 & $^{\theta}$$^{\kappa}$\UseMacro{result-CG_CP_RNNBaseline_test_standard_exact_match}
 & \UseMacro{result-CG_T_RNNBaseline_val_exact_match}
 & \UseMacro{result-CG_T_RNNBaseline_test_standard_exact_match}
\\
\UseMacro{TH-model-TransformerACL20}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_val_exact_match}}
 & \textbf{\UseMacro{result-CG_MP_TransformerACL20_test_standard_exact_match}}
 & $^{\eta}$\UseMacro{result-CG_CP_TransformerACL20_val_exact_match}
 & $^{\iota}$$^{\kappa}$\textbf{\UseMacro{result-CG_CP_TransformerACL20_test_standard_exact_match}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_val_exact_match}}
 & \textbf{\UseMacro{result-CG_T_TransformerACL20_test_standard_exact_match}}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-CG}}
\caption{\UseMacro{TC-results-aux-CG}}
\end{table}


==> tables/table-results-aux-MN.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{footnotesize}
\begin{center}
\begin{tabular}{@{\hspace{0pt}} l @{\hspace{0pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r@{\hspace{2pt}} | r@{\hspace{2pt}} | @{\hspace{2pt}}r @{\hspace{0pt}}}
\toprule
\makecell[c]{\UseMacro{TH-train-on}}
 & \multicolumn{2}{c|}{\UseMacro{TH-MP}}
 & \multicolumn{2}{c|}{\UseMacro{TH-CP}}
 & \multicolumn{2}{c}{\UseMacro{TH-T}}
\\ \cline{2-3} \cline{4-5} \cline{6-7}
\makecell[c]{\UseMacro{TH-test-on}}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
 & \UseMacro{TH-val}
 & \UseMacro{TH-test_standard}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_p}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_p}}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_p}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_p}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_p}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_p}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_p}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_p}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_p}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_p}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_p}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_p}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_p}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_r}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_r}}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_r}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_r}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_r}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_r}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_r}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_r}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_r}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_r}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_r}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_r}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_r}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-set_match_f}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_val_set_match_f}}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_set_match_f}}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_val_set_match_f}
 & \UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_set_match_f}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_val_set_match_f}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_set_match_f}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_set_match_f}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_set_match_f}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_val_set_match_f}}
 & \textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_set_match_f}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_set_match_f}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_set_match_f}
\\
\midrule
\midrule
\multicolumn{7}{c}{\UseMacro{TH-metric-table-exact_match}} \\
\midrule
\UseMacro{TH-model-Code2VecPOPL19}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_val_exact_match}}
 & \textbf{\UseMacro{result-MN_MP_Code2VecPOPL19_test_standard_exact_match}}
 & $^{\alpha}$\UseMacro{result-MN_CP_Code2VecPOPL19_val_exact_match}
 & $^{\beta}$\UseMacro{result-MN_CP_Code2VecPOPL19_test_standard_exact_match}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_val_exact_match}}
 & \textbf{\UseMacro{result-MN_T_Code2VecPOPL19_test_standard_exact_match}}
\\
\UseMacro{TH-model-Code2SeqICLR19}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_val_exact_match}
 & \UseMacro{result-MN_MP_Code2SeqICLR19_test_standard_exact_match}
 & $^{\alpha}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_val_exact_match}}
 & $^{\beta}$\textbf{\UseMacro{result-MN_CP_Code2SeqICLR19_test_standard_exact_match}}
 & \UseMacro{result-MN_T_Code2SeqICLR19_val_exact_match}
 & \UseMacro{result-MN_T_Code2SeqICLR19_test_standard_exact_match}
\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\vspace{\UseMacro{TV-results-aux-MN}}
\caption{\UseMacro{TC-results-aux-MN}}
\end{table}


==> tikz/use-case.tex <==
% \documentclass{standalone}

% \RequirePackage[T1]{fontenc}
% \RequirePackage[tt=false, type1=true]{libertine}
% \RequirePackage[varqu]{zi4}
% \RequirePackage[libertine]{newtxmath}

% \usepackage{hyperref}
% \input{macros}

% \begin{document}

\begin{tikzpicture}[
  line width=0.4pt,
  node distance=0ex and 0em,
  every node/.style={scale=0.9},
  gridBox/.style={rectangle, opacity=0, draw=red},
  box/.style={rectangle, draw=black, inner sep=3pt, font=\small, text depth=.25ex, text height=1.25ex},
  rounded box/.style={box, rounded corners, draw=black, inner sep=3pt, font=\small},
  anno/.style={font=\footnotesize},
]

  \tikzset{
    bg box/.style={box, draw=none, fill=black!10, inner sep=2pt, font=\footnotesize},
  }
  
  \node (b-task) at (0, 0) [rounded box] {Formalize Task};
  \node (c-examples) at (4em, 0) [coordinate] {};

  \node (b-task-cg) at (b-task.east -| c-examples) [anchor=west, bg box] {\comgen};
  \node (b-task-mn) [right = .1em of b-task-cg] [bg box] {\metnam};
  \node (b-task-others) [right = .1em of b-task-mn] [bg box] {$\cdots$};

  \node (b-use-case) [below = 2ex of b-task] [rounded box, fill=red!10] {Describe Use Case};

  \node (b-uc-mixedproj) at (b-use-case.east -| c-examples) [anchor=west, yshift=1ex, bg box] {\ipmode};
  \node (b-uc-crossproj) [below right = 1.2ex and -3em of b-uc-mixedproj.east] [bg box] {\pmode};
  \node (b-uc-temporal) [above right = 1.2ex and -2em of b-uc-crossproj.east] [bg box] {\cmode};
  \node (b-uc-others) [below right = 1.2ex and -.5em of b-uc-temporal.east] [bg box] {$\cdots$};

  \node (b-methodology) [below = 2ex of b-use-case] [rounded box] {Select \Methodology};

  \node (b-m-mixedproj) at (b-methodology.east -| c-examples) [anchor=west, bg box] {\mixedproj};
  \node (b-m-crossproj) [right = .1em of b-m-mixedproj] [bg box] {\crossproj};
  \node (b-m-temporal) [right = .1em of b-m-crossproj] [bg box] {\temporal};
  \node (b-m-others) [right = .1em of b-m-temporal] [bg box] {$\cdots$};

  \node (b-train) [below = 2ex of b-methodology] [rounded box] {Train Model};

  \node (b-eval) [below = 2ex of b-train] [rounded box] {Evaluate Model};

  \draw[->, thick] (b-task) to (b-use-case);
  \draw[->, thick] (b-use-case) to (b-methodology);
  \draw[->, thick] (b-methodology) to (b-train);
  \draw[->, thick] (b-train) to (b-eval);

  \draw[->, draw=black!50] (b-uc-mixedproj) to (b-m-mixedproj);
  \draw[->, draw=black!50] (b-uc-crossproj) to (b-m-crossproj);
  \draw[->, draw=black!50] (b-uc-temporal) to (b-m-temporal);

\end{tikzpicture}

% \end{document}

